Dualization of the Hopf algebra of secondary cohomology operations and the Adams spectral sequence

We describe the dualization of the algebra of secondary cohomology operations in terms of generators extending the Milnor dual of the Steenrod algebra. In this way we obtain explicit formulae for the computation of the E_3-term of the Adams spectral sequence converging to the stable homotopy groups of spheres.

==> dHascoAss_c8s.tex <==
\chapter{Computation of the algebra of secondary cohomology operations and its
dual}\label{A}

We first describe explicit splittings of the pair algebra $\R^\FF$ of relations
in the Steenrod algebra and its dual $\R_\FF$. Then we describe in terms of
these splittings $s$ the multiplication maps $A^s$ for the Hopf pair algebra
$\aB^\FF$ of secondary cohomology operations and we describe the dual maps
$A_s$ determining the Hopf pair coalgebra $\aB_\FF$ dual to $\aB^\FF$. On the
basis of the main result in the book \cite{Baues} we describe systems of
equations which can be solved inductively by a computer and which yield the
multiplication maps $A^s$ and $A_s$ as a solution. It turns out that $A_s$ is
explicitly given by a formula in which only the values $A_s(\zeta_n)$,
$n\ge1$, have to be computed where $\zeta_n$ is the Milnor generator in the
dual Steenrod algebra $\A_*$.

\section{Computation of $\R^\FF$ and $\R_\FF$}\label{rcomp}

Let us fix a function $\chi:\FF\to\GG$ which splits the projection
$\GG\to\FF$, namely, take
\begin{equation}\label{chieq}
\chi(k\!\!\mod p) = k\!\!\mod p^2, \ 0\le k<p.
\end{equation}
We will use $\chi$ to define splittings of
$\R^\FF=\left(\R^\FF_1\xto\d\R^\FF_0\right)$. Here a \emph{splitting} $s$
of $\R^\FF$ is an $\FF$-linear map for which the diagram
\begin{equation}\label{s}
\alignbox{
\xymatrix{
&&\R^\FF_1\ar[d]^\d\\
R_\F\ar@{ (->}[r]\ar[urr]^s
&\F_0\ar@{=}[r]
&\R^\FF_0
}
}
\end{equation}
commutes with $R_\F=\im(\d)=\ker(q_\F:\F_0\to\A)$. We only consider the
case $p=2$.

\begin{Definition}[The right equivariant splitting of $\R^\FF$]\label{chi}
Using $\chi$, all \emph{Adem relations}
$$
[a,b]:=\Sq^a\Sq^b+\sum_{k=0}^{\left[\frac
a2\right]}\binom{b-k-1}{a-2k}\Sq^{a+b-k}\Sq^k
$$
for $a,b>0$, $a<2b$, can be lifted to elements $[a,b]_\chi\in R_\aB$ by
applying $\chi$ to all coefficients, i.~e. by interpreting $[a,b]$ as an
element of $\aB$. As shown in \cite{Baues}*{16.5.2}, $R_\F$ is a free right
$\F_0$-module with a basis consisting of \emph{preadmissible relations}. For
$p=2$ these are elements of the form
$$
\Sq^{a_1}\cdots\Sq^{a_{k-1}}[a_k,a]\in R_\F
$$
satisfying $a_1\ge2a_2$, ..., $a_{k-2}\ge2a_{k-1}$, $a_{k-1}\ge2a_k$,
$a_k<2a$. Sending such an element to
$$
\Sq^{a_1}\cdots\Sq^{a_{k-1}}[a_k,a]_\chi\in R_\B
$$
determines then a unique right $\F_0$-equivariant splitting $\phi$ in the pair
algebra $\R^\FF$; that is, we get a commutative diagram
$$
\xymatrix@!C=5em{
R_\F\ar[r]^-\phi\ar@{ (->}[d]
&**[l]R_\aB\ox\FF=\R^\FF_1\ar[d]^\d\\
\F_0\ar@{=}[r]
&\R^\FF_0.
}
$$
\end{Definition}

For a splitting $s$ of $\R^\FF$ the map $s\!\ox\!1\oplus1\!\ox\!s$
induces the map $s_\#$ in the diagram
\begin{equation}\label{rsplit}
\alignbox{
\xymatrix{
\R^\FF_1\ar[r]^-\Delta\ar@{->>}[d]^\d
&(\R^\FF\hat\ox\R^\FF)_1\ar@{->>}[d]^{\d_{\hat\ox}}
&\R^\FF_1\!\ox\!\F_0\oplus\F_0\!\ox\!\R^\FF_1\ar[l]\\
R_\F\ar@/^/@{-->}[u]^s\ar@{ (->}[d]\ar[r]^{\Delta_R}
&R^{(2)}_\F\ar@/^/@{-->}[u]^{s_\#}\ar@{ (->}[d]
&R_\F\!\ox\!\F_0\oplus\F_0\!\ox\!R_\F\ar[l]\ar@{-->}[u]_{s\ox\!1\oplus1\!\ox\!s}\\
\F_0\ar[r]^-\Delta
&\F_0\ox\F_0.
}
}
\end{equation}
Then the difference
$U=s_\#\Delta_R-\Delta s:R_\F\to(\R^\FF\hat\ox\R^\FF)_1$ satisfies $\d_{\hat\ox}U=0$ since
$$
\d_{\hat\ox} s_\#\Delta_R=\Delta_R=\Delta_R\d s=\d_{\hat\ox}\Delta s.
$$
Thus $U$ lifts to $\ker\d_{\hat\ox}\cong\A\ox\A$ and gives an $\FF$-linear
map
\begin{equation}\label{ueq}
U^s:R_\F\to\A\ox\A.
\end{equation}
If we use the splitting $s$ to identify $\R^\FF_1$ with the direct sum
$\A\oplus R_\F$, then it is clear that knowledge of the map $U^s$ determines the
diagonal $\R^\FF_1\to(\R^\FF\hat\ox\R^\FF)_1$ completely. Indeed $s_\#$
yields the identification $(\R^\FF\hat\ox\R^\FF)_1\cong\A\!\ox\!\A\oplus
R^{(2)}_\F$, and under these identifications
$\Delta:\R^\FF_1\to(\R^\FF\hat\ox\R^\FF)_1$ corresponds to a map which by
commutativity of \eqref{rsplit} must have the form
\begin{equation}\label{udia}
\A\oplus R_\F
\xto{\left(\begin{smallmatrix}\Delta_\A&U^s\\0&\Delta_R\end{smallmatrix}\right)}
\A\!\ox\!\A\oplus R^{(2)}_\F
\end{equation}
and is thus determined by $U^s$.

One readily checks that the map $U^s$ for $s=\phi$ in \bref{chi} coincides with the map $U$
defined in \cite{Baues}*{16.4.3} in terms of the algebra $\aB$.

Given the splitting $s$ and the map $U^s$, the only piece of structure
remaining to determine the $\Alg^\pair_\oo$-comonoid structure of
$\R^\FF$ completely is the $\F_0$-$\F_0$-bimodule structure on
$\R^\FF_1\cong\A\oplus R_\F$. Consider for $f\in\F_0$, $r\in R_\F$ the
difference $ s(fr)-f s(r)$. It belongs to the kernel of $\d$ since
$$
\d s(fr)=fr=f\d s(r)=\d(f s(r)).
$$
Thus we obtain the \emph{left multiplication map}
\begin{equation}\label{aeq}
a^s:\F_0\ox R_\F\to\A.
\end{equation}

Similarly we obtain the \emph{right multiplication map}
$$
b^s:R_\F\ox\F_0\to\A
$$
by the difference $s(rf)-s(r)f$.

\begin{Lemma}\label{chisp}
For $s=\phi$ in \bref{chi} the right multiplication map $b^\phi$ is trivial,
that is $\phi$ is right equivariant, and the left multiplication map factors
through $q_\F\ox1$ inducing the map
$$
a^\phi:\A\ox R_\F\to\A.
$$
\end{Lemma}

\begin{proof}
Right equivariance holds by definition. As for the factorization, $R_\F\ox
R_\F\into\F_0\ox R_\F$ is in the kernel of $a^\phi:\F_0\ox R_\F\to\A$, since
by right equivariance of $s$ and by the pair algebra property \eqref{paireq}
for $\R^\FF$ one has for any $r,r'\in R_\F$
$$
s(rr')=s(r)r'=s(r)\d s(r')=(\d s(r))s(r')=rs(r').
$$
Hence factoring the above map through $(\F_0\ox R_\F)/(R_\F\ox
R_\F)\cong\A\ox R_\F$ we obtain a map
$$
\A\ox R_\F\to\A.
$$
\end{proof}

Summarizing the above, we thus have proved

\begin{Proposition}\label{detrel}
Using the splitting $s=\phi$ of $\R^\FF$ in \bref{chi}
the comonoid $\R^\FF$ in the category $\Alg^\pair_\oo$ described
in \bref{relcom} is completely determined by the maps
$$
U^\phi:R_\F\to\A\ox\A
$$
and
$$
a^\phi:\A\ox R_\F\to\A
$$
given in \eqref{ueq} and \eqref{aeq} respectively.
\end{Proposition}\qed

We next introduce another splitting $s=\psi$ for which $U^s=0$. For this we use
the fact that $\A_*=\Hom(\A,\FF)$ and
\begin{equation}
\aB_\#=\Hom(\aB_0,\GG)
\end{equation}
with $\aB_0=T_\GG(E_\A)$ both are polynomial algebras in such a way that
generators of $\A_*$ are also (part of the) generators of $\aB_\#$.

Using $\chi$ in \eqref{chieq} we obtain the function
\begin{equation}\label{psichi}
\psi_\chi:\A_*\to\aB_\#
\end{equation}
(which is not $\FF$-linear) as follows. Each element $x$ in $\A_*$ is
uniquely an $\FF$-linear combination $x=\sum_\alpha n_\alpha\alpha$ where
$\alpha$ runs through the monomials in Milnor generators. Such a monomial
can be also considered as an element in $\aB_\#$ by \bref{eslp} so that we
can define
$$
\psi_\chi(x)=\sum_\alpha\chi(n_\alpha)\alpha\in\aB_\#.
$$

\begin{Definition}[The comultiplicative splitting of $\R^\FF$]\label{psi}
Consider the following commutative diagram with exact rows and columns
$$
\xymatrix{
\A_*\ar@{ >->}[r]\ar@{-->}[dr]_{\psi_\chi}&\F_*\ar[r]&\Hom(R_\aB,\FF)\\
&\aB_\#\ar[r]^-q\ar@{->>}[u]&\Hom(R_\aB,\GG)\ar[u]\\
\A_*\ar@{ >->}[r]^{{q_\F}_*}&\F_*\ar@{ >->}[u]_j\ar[r]
&\Hom(R_\aB,\FF)\ar@{ >->}[u]_{j_R}\ar@{->>}[r]&\A_*\ar@{-->}[dl]^{q\psi_\chi}\\
&\R_\FF^0\ar@{=}[u]&\R_\FF^1\ar@{=}[u]
}
$$
with the columns induced by the short exact sequence $\FF\into\GG\onto\FF$
and the rows induced by \eqref{drel}. In particular $q$ is induced by the
inclusion $R_\aB\subset\aB_0$. Now it is clear that $\psi_\chi$ yields a map
$q\psi_\chi$ which lifts to $\Hom(R_\aB,\FF)$ so that we get the map
$$
q\psi_\chi:\A_*\to\R_\FF^1
$$
which splits the projection $\R_\FF^1\onto\A_*$. Moreover $q\psi_\chi$ is
$\FF$-linear since for all $x,y\in\A_*$ the elements
$\psi_\chi(x)+\psi_\chi(y)-\psi_\chi(x+y)\in\aB_\#$ are in the image of the
inclusion $j{q_\F}_*:\A_*\into\aB_\#$ and thus go to zero under $q$.

The dual of $q\psi_\chi$ is thus a retraction $(q\psi_\chi)^*$ in the
short exact sequence
$$
\xymatrix{
R_\F\ar@{-->}[dr]_{(q\psi_\chi)^*_\perp}&R_\aB\ox\FF\ar@{=}[d]\ar@{->>}[l]_\pi&\A\ar@{
>->}[l]_-\iota\\
&\R^\FF_1\ar@{-->}[ur]_{(q\psi_\chi)^*}
}
$$
which induces the splitting $\psi=(q\psi_\chi)^*_\perp$ of $\R^\FF$
determined by
$$
\psi(\pi(x))=x-\iota((q\psi_\chi)^*(x)).
$$
\end{Definition}

\begin{Lemma}
For the splitting $s=\psi$ of $\R^\FF$ we have $U^\psi=0$.
\end{Lemma}

\begin{proof}
We must show that the following diagram commutes:
$$
\xymatrix{
R_\F\ar[r]^{\Delta_R}\ar[d]_\psi&R_\F^{(2)}\ar[d]^{\psi_\#}\\
R_\aB\ox\FF\ar[r]^-\Delta&(\R^\FF\hat\ox\R^\FF)_1.
}
$$
Obviously this is equivalent to commutativity of the dual diagram
$$
\xymatrix{
(\R_\FF\check\ox\R_\FF)^1\ar[r]^-{\Delta_*}\ar[d]_{(\psi_\#)_*}&\Hom(R_\aB,\FF)\ar[d]^{\psi_*}\\
{R_\F^{(2)}}_*\ar[r]^{{\Delta_R}_*}&{R_\F}_*
}
$$
which in turn is equivalent to commutativity of
\begin{equation}\label{psicom}
\alignbox{
\xymatrix{
\A_*\ox\A_*\ar[d]_{(\psi_\#)_*^\perp}\ar[r]^{\delta_*}&\A_*\ar[d]^{q\psi_\chi}\\
(\R_\FF\check\ox\R_\FF)^1\ar[r]^-{\Delta_*}&\Hom(R_\aB,\FF).
}
}
\end{equation}
On the other hand, the left hand vertical map in the latter diagram can be
included into another commutative diagram
$$
\xymatrix{
\F_*\!\ox\!\A_*\oplus\A_*\!\ox\!\F_*
\ar[d]_{1\!\ox\!q\psi_\chi\oplus q\psi_\chi\!\ox\!1}
&\A_*\ox\A_*
\ar@{ )->}[l]_-{\binom{i\ox1}{1\ox i}}\ar[d]^{(\psi_\#)_*^\perp}\\
\F_*\!\ox\!\R_\FF^1\oplus\R_\FF^1\!\ox\!\F_*&(\R_\FF\ox\R_\FF)^1\ar@{ )->}[l]
}
$$
It follows that on elements, commutativity of \eqref{psicom} means that the
equality
$$
q\psi_\chi(xy)=i(x)q\psi_\chi(y)+q\psi_\chi(x)i(y)
$$
holds for any $x,y\in\A_*$. By linearity, it is clearly enough to prove
this when $x$ and $y$ are monomials in Milnor generators.

For this observe that for any $x\in\A_*=\Hom(\A,\FF)$, the element
$q\psi_\chi(x)\in\Hom(R_\aB,\FF)$ is the unique $\FF$-linear map making the
diagram
$$
\xymatrix{
R_\aB\ar@{ >->}[r]\ar@{-->}[d]_{q\psi_\chi(x)}
&\aB_0\ar[d]_{\psi_\chi(x)}\ar@{->>}[r]
&\A\ar[d]^x\\
\FF\ar@{ >->}[r]
&\GG\ar@{->>}[r]
&\FF
}
$$
commute. This uniqueness implies the equality we need in view of the
following commutative diagram with exact columns:
$$
\xymatrix@!C=5em{
R_\aB\ar[r]\ar@{ >->}[d]
&R_\aB^{(2)}\ar@{ >->}[d]\ar@{-->}[r]
&\FF\ox\FF\ar[r]^\cong\ar@{ >->}[d]
&\FF\ar@{ >->}[d]\\
\aB_0\ar[r]^-\Delta\ar@{->>}[d]
&\aB_0\ox\aB_0\ar@{->>}[d]\ar[r]^{\psi_\chi(x)\ox\psi_\chi(y)}
&\GG\ox\GG\ar@{->>}[d]\ar[r]^\cong
&\GG\ar@{->>}[d]\\
\A\ar[r]^-\delta\ar@/_3ex/[rrr]_{xy}
&\A\ox\A\ar[r]^{x\ox y}
&\FF\ox\FF\ar[r]^\cong
&\FF,
}
$$
since when $x$ and $y$ are monomials in Milnor generators, one has
$\psi_\chi(xy)=\psi_\chi(x)\psi_\chi(y)$. 
\end{proof}

Therefore we call $\psi$ the comultiplicative splitting of $\R^\FF$. We now
want to compute the left and right multiplication maps $a^\psi$ and
$b^\psi$ defined in \eqref{aeq}. The dual maps $a_\psi=(a^\psi)_*$ and
$b_\psi=(b^\psi)_*$ can be described by the diagrams
\begin{equation}\label{ml}
\alignbox{
\xymatrix{
&(R_\aB)_*\ar@{->>}[r]\ar[d]_{m_*^\l}&\A_*\ar@/_1em/@{-->}[l]_{q\psi_\chi}\ar[d]^{m_*}\\
\F_*\ox(R_\F)_*\ar@{
(->}[r]&\F_*\ox(R_\aB)_*\ar@{->>}[r]
&\A_*\ox\A_*\ar@/^1em/@{-->}[l]^{i\ox q\psi_\chi}
}
}
\end{equation}
and
\begin{equation}\label{mr}
\alignbox{
\xymatrix{
&(R_\aB)_*\ar@{->>}[r]\ar[d]_{m_*^\r}&\A_*\ar@/_1em/@{-->}[l]_{q\psi_\chi}\ar[d]^{m_*}\\
(R_\F)_*\ox\F_*\ar@{
(->}[r]&(R_\aB)_*\ox\F_*\ar@{->>}[r]
&\A_*\ox\A_*.\ar@/^1em/@{-->}[l]^{q\psi_\chi\ox i}
}
}
\end{equation}
Here $m_*$ is dual to the multiplication in $\A$ and $m_*^\l$ and $m_*^\r$
are induced by the $\F_0$-$\F_0$-bimodule structure of $R_\aB\ox\FF$. One
readily checks
\begin{align*}
a_\psi&=m_*^\l q\psi_\chi-(i\ox q\psi_\chi)m_*\\
b_\psi&=m_*^\r q\psi_\chi-(q\psi_\chi\ox i)m_*.
\end{align*}
We now consider the diagram
$$
\xymatrix{
&\aB_\#\ar[d]_{m_*^\GG}&\A_*\ar[l]_{\psi_\chi}\ar[d]^{m_*}\\
\F_*\ox\F_*\ar@{ (->}[r]&\aB_\#\ox\aB_\#&\A_*\ox\A_*\ar[l]_-{\psi_\chi^\ox}
}
$$
Here $\psi_\chi^\ox$ is defined similarly as $\psi_\chi$ in \eqref{psichi}
by the formula
$$
\psi_\chi^\ox\left(\sum_{\alpha,\beta}n_{\alpha\beta}\alpha\ox\beta\right)=
\sum_{\alpha,\beta}\chi(n_{\alpha\beta})\alpha\ox\beta
$$
where $\alpha$, $\beta$ run through the monomials in Milnor generators.
Moreover $m_*^\GG$ is the dual of the multiplication map $m^\GG$ of
$\aB_0=T_\GG(E_\A)$.

\begin{Lemma}\label{mulstar}
The difference $m^\GG_*\psi_\chi-\psi_\chi^\ox m_*$ lifts to an
$\FF$-linear map $\nabla_\chi:\A_*\to\F_*\ox\F_*$ such that one has
\begin{align*}
a_\psi&=(1\ox\pi)\nabla_\chi\\
b_\psi&=(\pi\ox1)\nabla_\chi.
\end{align*}
Here $\pi:\F_*\onto{R_\F}_*$ is induced by the inclusion $R_\F\subset\F_0$.
\end{Lemma}

\begin{proof}
We will only prove the first equality; the proof for the second one is
completely similar.

The following diagram
$$
\xymatrix@!C=3em{
&{R_\aB}_*\ar@{ >->}[rrd]_{j_R}\ar[ddddd]_{m^\l_*}&&&&&&\A_*\ar[llllll]_{q\psi_\chi}\ar@{=}[ddl]\ar[ddddd]^{m_*}\\
&&&{R_\aB}_\#\ar[ddd]_{m^\l_\#}\\
&&&&&\aB_\#\ar[d]_{m_*^\GG}\ar[ull]^\pi&\A_*\ar[l]_{\psi_\chi}\ar[d]^{m_*}\\
&&&&&\aB_\#\ox\aB_\#\ar[dll]_{1\ox\pi}&\A_*\ox\A_*\ar[l]_-{\psi_\chi^\ox}\\
&&&\aB_\#\ox{R_\aB}_\#&\F_*\ox\F_*\ar[lllldd]|\hole^>(.75){1\ox\pi}\ar@{ (->}[ur]\\
&\F_*\ox{R_\aB}_*\ar@{ >->}[urr]^{j\ox j_R}&&&&&&\A_*\ox\A_*\ar[llllll]^{i\ox q\psi_\chi}\ar@{=}[uul]\\
\F_*\ox{R_\F}_*\ar@{ (->}[ur]
}
$$
commutes except for the innermost square, whose deviation from
commutativity is $\nabla_\chi$ and lies in the image of
$\F_*\ox\F_*\incl\aB_\#\ox\aB_\#$, and the outermost square, whose deviation
from commutativity is $a_\psi$ and lies in the image of
$\F_*\ox{R_\F}_*\incl\F_*\ox{R_\aB}_*$. It follows that
$(1\ox\pi)\nabla_\chi$ and $a_\psi$ have the same image under $j\ox
j_R$, and since the latter map is injective we are done.
\end{proof}

Let us describe the map $\nabla_\chi$ more explicitly.

\begin{Lemma}
The map $\nabla_\chi$ factors as follows
$$
\A_*\xto{\bar\nabla\chi}\F_*\ox\A_*\xto{1\ox i}\F_*\ox\F_*.
$$
\end{Lemma}

\begin{proof}
Let $\A_\#\subset\aB_\#$ be the subring generated by the elements $M_1$,
$M_{21}$, $M_{421}$, $M_{8421}$, .... It is then clear that the image of
$\psi_\chi$ lies in $\A_\#$ and the reduction $\aB_\#\onto\F_*$ carries
$\A_\#$ to $\A_*$. Moreover obviously the image of $\psi^\ox m_*$ lies in
$\A_\#$, hence it only remains to show the inclusion
$$
m_*^\GG(\A_\#)\subset\aB_\#\ox\A_\#.
$$
Since $m_*^\GG$ is a ring homomorphism, it suffices to check this on the
generators $M_1$, $M_{21}$, $M_{421}$, $M_{8421}$, .... But this is clear from
\eqref{dizeta}.
\end{proof}

\begin{Corollary}\label{calcab}
For the comultiplicative splitting $\psi$ one has
$$
a_\psi=0.
$$
Moreover the map $b_\psi$ factors as follows
$$
\A_*\xto{\bar b_\psi}{R_\F}_*\ox\A_*\xto{1\ox i}{R_\F}_*\ox\F_*.
$$
\end{Corollary}

\begin{proof}
The first statement follows as by definition $\pi(\A_*)=0$; the second is
obvious.
\end{proof}

Using the splitting $\psi$ we get the following analogue of \bref{detrel}.

\begin{Proposition}\label{psicomon}
The comonoid $\R^\FF$ in the category $\Alg^\pair_\oo$ described in
\bref{relcom} is completely determined by the multiplication map
$$
\bar b^\psi: R_\F\ox\A\to\A
$$
dual to the map $\bar b_\psi$ from \ref{calcab}. In fact, the identification
$$
\R^\FF_1=\A\oplus R_\F
$$
induced by the splitting $s=\psi$ identifies the diagonal of $\R^\FF$ with
$\Delta_\A\oplus\Delta_R$ (see \eqref{ueq}, \eqref{udia}), and the bimodule
structure of $\R_1^\FF$ with
\begin{align*}
f(\alpha,r)&=(f\alpha,fr)\\
(\alpha,r)f&=(\alpha\qf f-\bar b^\psi(r,\qf f),rf)
\end{align*}
for $f\in\F_0$, $r\in R_\F$, $\alpha\in\A$.
\end{Proposition}

\section{Computation of the Hopf pair algebra $\aB^\FF$}\label{bcomp}

The Hopf pair algebra $\V=\aB^\FF$ in \bref{unique}, given by the algebra of
secondary cohomology operations, satisfies the following crucial condition
which we deduce from \cite{Baues}*{16.1.5}.

\begin{Theorem}\label{splitr}
There exists a right $\F_0$-equivariant splitting
$$
u:\R^\FF_1=R_\aB\ox\FF\to\aB_1\ox\FF=\aB^\FF_1
$$
of the projection $\aB^\FF_1\to\R^\FF_1$, see \eqref{hpad}, such that the
following holds. The diagram
$$
\xymatrix{
\A\oplus_\k\Sigma\A\ar@/_/@{-->}[d]_q\ar@{ >->}[r]
&\aB^\FF_1\ar@/_/@{-->}[d]_q\ar[r]
&\aB^\FF_0\ar@{=}[d]\ar@{->>}[r]
&\A\ar@{=}[d]\\
\A\ar[u]_{\bar u}\ar@{ >->}[r]
&\R^\FF_1\ar[u]_u\ar[r]
&\R^\FF_0\ar@{->>}[r]
&\A
}
$$
commutes, where $\bar u$ is the inclusion. Moreover in the diagram of
diagonals, see \eqref{diacomp},
$$
\xymatrix{
\aB^\FF_1\ar[r]^-{\Delta_\aB}
&(\aB^\FF\hat\ox\aB^\FF)_1
&\Sigma\A\ox\A\ar@{ )->}[l]\\
\R^\FF_1\ar[r]^-{\Delta_R}\ar[u]^u
&(\R^\FF\hat\ox\R^\FF)_1\ar[u]^{u\hat\ox u}
}
$$
the difference $\Delta_\aB u-(u\hat\ox u)\Delta_R$ lifts to $\Sigma\A\ox\A$
and satisfies
$$
\xi\bar\pi=\Delta_\aB u-(u\hat\ox
u)\Delta_R:\xymatrix@1{\R_\FF^1\ar@{->>}[r]^{\bar\pi}&\bar
R\ar[r]^-\xi&\Sigma\A\ox\A}
$$
where $\xi$ is dual to $\xi_*$ in \bref{cosxi}. Here $\bar\pi$ is the
projection $\R_\FF\onto R_\F\onto\bar R$. The cocycle $\xi$ is trivial if
$p$ is odd.
\end{Theorem}

\begin{Definition}\label{multop}
Using a splitting $u$ of $\aB^\FF$ as in \bref{splitr} we define a
\emph{multiplication operator}
$$
A:\A\ox R_\aB\to\Sigma\A
$$
by the equation
$$
A(\bar\alpha\ox x)=u(\alpha x)-\alpha u(x)
$$
for $\alpha\in\F_0$, $x\in R_\aB$. Thus $-A$ is a multiplication map as
studied in \cite{Baues}*{16.3.1}. Fixing a splitting $s$ of $\R^\FF$ as in
\eqref{s} we define an \emph{$s$-multiplication operator} $A^s$ to be the
composite
$$
A^s:\xymatrix@1{\A\ox R_\F\ar[r]^-{1\ox s}&\A\ox R_\aB\ar[r]^-A&\Sigma\A}.
$$
Such operators have the properties of the following $s$-multiplication
maps.
\end{Definition}

\begin{Definition}\label{mulmap}
Let $s$ be a splitting of $\R^\FF$ as in \eqref{s} and let $U^s$, $a^s$,
$b^s$ be defined as in section \ref{rcomp}. An \emph{$s$-multiplication
map}
$$
A^s:\A\ox R_\F\to\A
$$
is an $\FF$-linear map of degree $-1$ satisfying the following conditions
with $\alpha,\alpha',\beta,\beta'\in\F_0$, $x,y\in R_\F$
\begin{enumerate}
\item $A^s(\alpha,x\beta)=A^s(\alpha,x)\beta+\k(\alpha)b^s(x,\beta)$
\item
$A^s(\alpha\alpha',x)=A^s(\alpha,\alpha'x)+\k(\alpha)a^s(\alpha',x)+(-1)^{\deg(\alpha)}\alpha
A^s(\alpha',x)$
\item $\delta A^s(\alpha,x)=A^s_\ox(\alpha\ox\Delta
x)+L(\alpha,x)+\nabla_\xi(\alpha,x)+\delta\k(\alpha)U^s(x)$.
\end{enumerate}
Here $A^s_\ox:\A\ox R_\F^{(2)}\to\A\ox\A$ is defined by the equalities
\begin{align*}
A^s_\ox(\alpha\ox x\ox\beta')
&=\sum(-1)^{\deg(\alpha_\r)\deg(x)}A^s(\alpha_\l,x)\ox\alpha_\r\beta',\\
A^s_\ox(\alpha\ox\beta\ox y)
&=\sum(-1)^{\deg(\alpha_\r)\deg(\beta)+\deg(\alpha_\l)+\deg(\beta)}\alpha_\l\beta\ox
A^s(\alpha_\r,y),
\end{align*}
where as always
$$
\delta(\alpha)=\sum\alpha_\l\ox\alpha_\r\in\A\ox\A.
$$

Two $s$-multiplication maps $A^s$ and ${A^s}'$  are \emph{equivalent} if there exists an
$\FF$-linear map
$$
\gamma:R_\F\to\A
$$
of degree $-1$ such that the equality
$$
A^s(\alpha,x)-{A^s}'(\alpha,x)
=\gamma(\alpha x)-(-1)^{\deg(\alpha)}\alpha\gamma(x)
$$
holds for any $\alpha\in\A$, $x\in R_\F$ and moreover $\gamma$ is right
$\F_0$-equivariant and the diagram
$$
\xymatrix{
\A\ar[r]^-\delta&\A\ox\A\\
R_\F\ar[u]_\gamma\ar[r]_\Delta&R_\F^{(2)}\ar[u]_{\gamma_\ox}
}
$$
commutes, with $\gamma_\ox$ given by
\begin{align*}
\gamma_\ox(x\ox\beta)&=\gamma(x)\ox\beta,\\
\gamma_\ox(\alpha\ox y)&=(-1)^{\deg(\alpha)}\alpha\ox\gamma(y)
\end{align*}
for $\alpha,\beta\in\F_0$, $x,y\in R_\F$.
\end{Definition}

\begin{Theorem}\label{exmul}
There exists an $s$-multiplication map $A^s$ and any two such
$s$-multiplication maps are equivalent. Moreover each $s$-multiplication
map is an $s$-multiplication operator as in \bref{multop} and vice versa.
\end{Theorem}

\begin{proof}
We apply \cite{Baues}*{16.3.3}. In fact, we obtain by $A^s$ the
multiplication operator
$$
A:\A\ox R_\aB=\A\!\ox\!\A\oplus\A\!\ox\!R_\F\to\Sigma\A
$$
with $A(\alpha\ox x)=A^s(\alpha\ox\bar x)+\k(\alpha)\xi$ where $(\bar
x,\xi)\in R_\F\oplus\A=R_\aB\ox\FF$ corresponds to $x$, that is $s(\bar
x)+\iota(\xi)=x$ for $\iota:\A\subset R_\aB\ox\FF$.
\end{proof}

\begin{Remark}
For the splitting $s=\phi$ of $\R^\FF$ in \bref{chi} the maps
$$
A_{n,m}:\A\to\A
$$
are defined by $A_{n,m}(\alpha)=A^\phi(\alpha\ox[n,m])$, with $[n,m]$
the Adem relations in $R_\F$. Using formul\ae\ in \bref{mulmap} the maps
$A_{n,m}$ determine the $\phi$-multiplication map $A^\phi$ completely. The
maps $A_{n,m}$ coincide with the corresponding maps $A_{n,m}$ in
\cite{Baues}*{16.4.4}. In \cite{Baues}*{16.6} an algorithm for
determination of $A_{n,m}$ is described, leading to a list of values of
$A_{n,m}$ on the elements of the admissible basis of $\A$. The algorithm
for the computation of $A_{n,m}$ can be deduced from theorem \bref{exmul}
above.
\end{Remark}

\begin{Remark}
Triple Massey products $\brk{\alpha,\beta,\gamma}$ with
$\alpha,\beta,\gamma\in\A$, $\alpha\beta=0=\beta\gamma$, as in \bref{tmp}
can be computed by $A^s$ as follows. Let $\bar\beta\bar\gamma\in R_\aB$ be
given as in \bref{tmp}. Then $\bar\beta\bar\gamma\ox1\in R_\aB\ox\FF$
satisfies
$$
\bar\beta\bar\gamma\ox1=s(\bar x)+\iota(\xi)
$$
with $\bar x\in R_\F$, $\xi\in\A$ and $\brk{\alpha,\beta,\gamma}$ satisfies
$$
A^s(\alpha\ox\bar x)+\k(\alpha)\xi\in\brk{\alpha,\beta,\gamma}.
$$
Compare \cite{Baues}*{16.3.4}.
\end{Remark}

Now it is clear how to introduce via $a^s$, $b^s$, $U^s$, $\xi$, $\k$, and $A^s$ a
Hopf pair algebra structure on
\begin{equation}\label{hopfin}
\alignbox{
\xymatrix{
\A\oplus\Sigma\A\oplus R_\F\ar[r]^-q\ar@{=}[d]&\A\oplus R_\F\ar@{=}[d]\\
\aB^\FF_1&\R^\FF_1
}
}
\end{equation}
which is isomorphic to $\aB^\FF$, compare \bref{detrel}.

In the next section we describe an algorithm for the computation of a
$\psi$-multiplication map, where $\psi$ is the comultiplicative splitting
of $\R^\FF$ in \bref{psi}. For this we compute the dual map $A_\psi$ of
$A^\psi$.

\section{Computation of the Hopf pair coalgebra $\aB_\FF$}\label{cobcomp}

For the comultiplicative splitting $s=\psi$ of $\R^\FF$ in \bref{psi} we
introduce the following $\psi$-comultiplication maps which are dual to the
$\psi$-multiplication maps in \bref{mulmap}.

\begin{Definition}\label{apsi}
Let $\bar b_\psi$ be given as in \ref{calcab}. A
\emph{$\psi$-comultiplication map}
$$
A_\psi:\A_*\to\A_*\ox{R_\F}_*
$$
is an $\FF$-linear map of degree $+1$ satisfying the following conditions.
\begin{enumerate}
\item\label{mreqs}
The maps in the diagram
$$
\xymatrix{
\A_*\ox{R_\F}_*\ar[d]_{1\ox m^\r_*}&\A_*\ar[d]^{m_*}\ar[l]_-{A_\psi}\\
\A_*\ox{R_\F}_*\ox\F_*&\A_*\ox\A_*\ar[l]^-{A_\psi\ox i}
}
$$
satisfy
$$
(1\ox m^\r_*)A_\psi=(A_\psi\ox i)m_*+(\k_*\ox\bar b_\psi)m_*.
$$
Here $\k_*$ is computed in \bref{dkappa} and $m^\r_*$ is defined in
\eqref{mr}.
\item\label{mleqs}
The maps in the diagram
$$
\xymatrix{
\A_*\ox{R_\F}_*\ar[d]^{1\ox m^\l_*}&&\A_*\ar[d]^{A_\psi}\ar[ll]_{A_\psi}\\
\A_*\ox\F_*\ox{R_\F}_*&\A_*\ox\A_*\ox{R_\F}_*\ar[l]^{1\ox i\ox1}
&\A_*\ox{R_\F}_*\ar[l]^-{m_*\ox1}
}
$$
satisfy
$$
(1\ox m^\l_*)A_\psi=(1\ox i\ox1)(m_*\ox1)A_\psi-(\tau\ox i\ox1)(1\ox A_\psi)m_*.
$$
Here $m^\l_*$ is as in \eqref{ml}, and $\tau:\A_*\to\A_*$ is given
by $\tau(\alpha)=(-1)^{\deg(\alpha)}\alpha$.
\item\label{mult}
For $x,y\in\A_*$ the product $xy$ in the algebra $\A_*$ satisfies the
formula
$$
A_\psi(xy)=A_\psi(x)m_*(y)+(-1)^{\deg(x)}m_*(x)A_\psi(y)+L_*(x,y)+{\nabla_\xi}_*(x,y).
$$
Here $L_*$ and ${\nabla_\xi}_*$ are given in \ref{L} and
\ref{nablaelts} respectively, with $L_*={\nabla_\xi}_*=0$ for $p$ odd.
\end{enumerate}

Two $\psi$-comultiplication maps $A_\psi$, $A_\psi'$ are
\emph{equivalent} if there is a derivation
$$
\gamma_*:\A_*\to{R_\F}_*
$$
of degree $+1$ satisfying the equality
$$
A_\psi-A_\psi'=m^\l_*\gamma_*-(\tau\ox\gamma_*)m_*.
$$
\end{Definition}

As a dual statement to \bref{exmul} we get

\begin{Theorem}
There exists a $\psi$-comultiplication map $A_\psi$ and any two such
$\psi$-comultiplication maps are equivalent. Moreover each
$\psi$-comultiplication map $A_\psi$ is the dual of a $\psi$-multiplication
map $A^\psi$ in \bref{exmul} with $A_\psi={A^\psi}_*$.
\end{Theorem}\qed

Now dually to \eqref{hopfin}, it is clear how to introduce via
$a_\psi$, $b_\psi$, $\xi_*$, $\k_*$, and $A_\psi$ a Hopf pair
coalgebra structure on
$$
\xymatrix{
\A_*\oplus\Sigma\A_*\oplus{R_\F}_*\ar@{=}[d]&\A_*\oplus{R_\F}_*\ar[l]_-i\ar@{=}[d]\\
\aB_\FF^1&\R_\FF^1
}
$$
which is isomorphic to $\aB_\FF$, compare \bref{psicomon}.

We now embark on the simplification and solution of the equations
\ref{apsi}\eqref{mreqs} and \ref{apsi}\eqref{mleqs}. To begin with, note that
the equations \ref{apsi}\eqref{mreqs} imply that the image of the composite
map
$$
\A_*\xto{A_\psi}\A_*\ox{R_\F}_*\xto{1\ox m^\r_*}\A_*\ox{R_\F}_*\ox\F_*
$$
actually lies in
$$
\A_*\ox{R_\F}_*\ox\A_*\subset\A_*\ox{R_\F}_*\ox\F_*;
$$
similarly \ref{apsi}\eqref{mleqs} implies that the image of
$$
\A_*\xto{A_\psi}\A_*\ox{R_\F}_*\xto{1\ox m^\l_*}\A_*\ox\F_*\ox{R_\F}_*
$$
lies in
$$
\A_*\ox\A_*\ox{R_\F}_*\subset\A_*\ox\F_*\ox{R_\F}_*.
$$

Now one obviously has

\begin{Lemma}
The following conditions on an element $x\in{R_\F}_*=\Hom(R_\F,\FF)$ are
equivalent:
\begin{itemize}
\item $m^\l_*(x)\in\A_*\ox{R_\F}_*\subset\F_*\ox{R_\F}_*$;
\item $m^\r_*(x)\in{R_\F}_*\ox\A_*\subset{R_\F}_*\ox\F_*$;
\item $x\in\bar R_*\subset{R_\F}_*$.
\end{itemize}
\end{Lemma}

\begin{proof}
Recall that $\bar R=R_\F/{R_\F}^2$, i.~e. $\bar R_*$ is the space of linear forms
on $R_\F$ which vanish on ${R_\F}^2$. Then the first condition means that
$x:R_\F\to\FF$ has the property that the composite
$$
\F_0\ox R_\F\xto{m^\l} R_\F\xto x\FF
$$
vanishes on $R_\F\ox R_\F\subset\F_0\ox R_\F$; but the image of $R_\F\ox R_\F$
under $m^\l$ is precisely ${R_\F}^2$. Similarly for the second condition.
\end{proof}

We thus conclude that the image of $A_\psi$ lies in $\A_*\ox\bar R_*$.

Next note that the condition \ref{apsi}\eqref{mult} implies
\begin{equation}\label{apsisq}
A_\psi(x^2)=L_*(x,x)+\nabla_{\xi_*}(x,x)
\end{equation}
for any $x\in\A_*$. Moreover the latter formula also implies

\begin{Proposition}\label{4=0}
For any $x\in\A_*$ one has
$$
A_\psi(x^4)=0.
$$
\end{Proposition}

\begin{proof}
Since the squaring map is an algebra endomorphism, by \ref{bider} one has
$$
L_*(x,y^2)=\sum\zeta_1x_\l y_{\l'}^2\ox\tilde L_*(x_r,y_{r'}^2),
$$
with
$$
m_*(x)=\sum x_\l\ox x_r,\ \ m_*(y)=\sum y_{\l'}\ox y_{r'}.
$$
But $\tilde L_*$ vanishes on squares since it is a biderivation, so $L_*$ also
vanishes on squares. Moreover by \eqref{nablaelts}
$$
\nabla_{\xi_*}(x^2,y^2)=\sum\xi_*(x^2,y^2)_\A\ox\xi_*(x^2,y^2)_R-\sum
x_\l^2y_{\l'}^2\ox\xi_*(x_r^2,y_{r'}^2);
$$
this is zero since $\xi_*(x^2,y^2)=0$ for any $x$ and $y$ by \eqref{xifromS}.
\end{proof}

Taking the above into account, and identifying the image of $i:\A_*\into\F_*$
with $\A_*$, \ref{apsi}\eqref{mreqs} can be rewritten as follows:
$$
(1\ox m_*^r)A_\psi(\zeta_n)
=A_\psi(\zeta_n)\ox1+\left(L_*(\zeta_{n-1},\zeta_{n-1})+\nabla_{\xi_*}(\zeta_{n-1},\zeta_{n-1})\right)\ox\zeta_1
+\sum_{i=0}^n\zeta_1\zeta_{n-i}^{2^i}\ox\bar b_\psi(\zeta_i),
$$
or
$$
(1\ox\tilde m_*^r)A_\psi(\zeta_n)
=\left(L_*(\zeta_{n-1},\zeta_{n-1})+\nabla_{\xi_*}(\zeta_{n-1},\zeta_{n-1})\right)\ox\zeta_1
+\sum_{i=0}^n\zeta_1\zeta_{n-i}^{2^i}\ox\bar b_\psi(\zeta_i).
$$
Still more explicitly one has
$$
L_*(\zeta_k,\zeta_k)=\sum_{0\le i,j\le k}\zeta_1\zeta_{k-i}^{2^i}\zeta_{k-j}^{2^j}\ox\tilde
L_*(\zeta_i,\zeta_j)=\sum_{0\le i\le k}\zeta_1\zeta_{k-i}^{2^{i+1}}\ox\tilde
L_*(\zeta_i,\zeta_i)
+\sum_{0\le i<j\le k}\zeta_1\zeta_{k-i}^{2^i}\zeta_{k-j}^{2^j}\ox\tilde
L^S_*(\zeta_i,\zeta_j),
$$
where we have denoted
$$
\tilde L^S_*(\zeta_i,\zeta_j):=\tilde
L_*(\zeta_i,\zeta_j)+\tilde L_*(\zeta_j,\zeta_i);
$$
similarly
$$
\nabla_{\xi_*}(\zeta_k,\zeta_k)=
\sum_{0\le i<j\le k}\zeta_{k-i}^{2^i}\zeta_{k-j}^{2^j}\ox
S_*(\zeta_i,\zeta_j).
$$
As for $b_\psi(\zeta_i)$, by \ref{mulstar} it can be calculated by the formula
\begin{equation}\label{bpsibar}
\bar b_\psi(\zeta_i)=\sum_{0<j<i}v_{i-j}^{2^{j-1}}\ox\zeta_j,
\end{equation}
where $v_k$ are determined by the equalities
$$
M_{2^k,2^{k-1},...,2}-M_{2^{k-1},2^{k-2},...,1}^2\equiv2v_k\mod4
$$
in $\aB_\#$. For example,
\begin{align*}
v_1&=M_{11},\\
v_2&=M_{411}+M_{231}+M_{222}+M_{2121},\\
v_3&
=M_{8411}
+M_{8231}
+M_{8222}
+M_{82121}
+M_{4631}
+M_{4622}
+M_{46121}
+M_{4442}
+M_{42521}
+M_{42431}
+M_{42422}\\
&+M_{424121}
+M_{421421},
\end{align*}
etc.

Thus putting everything together we see

\begin{Lemma}\label{mrC}
The equation \ref{apsi}\eqref{mreqs} for the
value on $\zeta_n$ is equivalent to
$$
(1\ox\tilde m^r_*)A_\psi(\zeta_n)=\sum_{0<k<n}C^{(n)}_{2^n-2^k+1}\ox\zeta_k
$$
where
\begin{multline*}
C^{(n)}_{2^n-1}=
\sum_{0<i<n}\zeta_1\zeta_{n-1-i}^{2^{i+1}}\ox\left(\tilde
L_*(\zeta_i,\zeta_i)+v_i\right)
+\sum_{0<i<j<n}\zeta_1\zeta_{n-1-i}^{2^i}\zeta_{n-1-j}^{2^j}\ox\tilde
L^S_*(\zeta_i,\zeta_j)
+\sum_{0<i<j<n}\zeta_{n-1-i}^{2^i}\zeta_{n-1-j}^{2^j}\ox
S_*(\zeta_i,\zeta_j)
\end{multline*}
and, for $1<k<n$,
$$
C^{(n)}_{2^n-2^k+1}=\sum_{0<i\le n-k}\zeta_1\zeta_{n-k-i}^{2^{k+i}}\ox
v_i^{2^{k-1}}.
$$
\end{Lemma}\qed

\begin{comment}
For low values of $n$ these equations look like
\begin{align*}
(1\ox\tilde m^r_*)A_\psi(\zeta_2)&=0,\\
(1\ox\tilde m^r_*)A_\psi(\zeta_3)&
=\zeta_1\ox(\pi(M_{222})\ox\zeta_1+\pi(M_{22})\ox\zeta_2)
+\zeta_1^2\ox\pi(M_{32}+M_{23}+M_{212}+M_{122})\ox\zeta_1\\
&+\zeta_1^3\ox\pi M_{22}\ox\zeta_1,\\
(1\ox\tilde m^r_*)A_\psi(\zeta_4)&
=\zeta_1\ox\left(\pi(M_{8222}+M_{722}+M_{4622}+M_{4442}+M_{42422})\ox\zeta_1\right.\\
&\ \ \ \ \ \ \ \left.+\pi(M_{822}+M_{462}+M_{444}+M_{4242})\ox\zeta_2+\pi(M_{44})\ox\zeta_3\right)\\
&+\zeta_1^4\ox\pi(M_{632}+M_{623}+M_{6212}+M_{6122}+M_{542}+M_{452}+M_{443}+M_{4412}+M_{4142}+M_{3422}\\
&\ \ \ \ \ \ \ +M_{2522}+M_{2432}+M_{2423}+M_{24212}+M_{24122}+M_{21422}+M_{1622}+M_{1442}+M_{12422})\ox\zeta_1\\
&+\zeta_1^5\ox\pi(M_{622}+M_{442}+M_{2422})\ox\zeta_1\\
&+\zeta_2^2\ox\pi(M_{522}+M_{432}+M_{423}+M_{4212}+M_{4122}+M_{1422})\ox\zeta_1
+\zeta_1\zeta_2^2\ox\pi(M_{422})\ox\zeta_1\\
&+\zeta_1^9\ox\left(\pi(M_{222})\ox\zeta_1+\pi(M_{22})\ox\zeta_2\right)
+\zeta_1^4\zeta_2^2\ox\pi(M_{32}+M_{23}+M_{212}+M_{122})\ox\zeta_1\\
&+\zeta_1^5\zeta_2^2\ox\pi(M_{22})\ox\zeta_1,
\end{align*}
etc. (Note that $A_\psi(\zeta_1)=0$ by dimension considerations.)

As for the equations \ref{apsi}\eqref{mleqs}, they have form
$$
(1\ox\tilde m^\l_*)A_\psi(\zeta_n)
=(\tilde m_*\ox1)A_\psi(\zeta_n)+\zeta_1^{2^{n-1}}\ox A_\psi(\zeta_{n-1})+\zeta_2^{2^{n-2}}\ox
A_\psi(\zeta_{n-2})+...+\zeta_{n-2}^4\ox A_\psi(\zeta_2)+\zeta_{n-1}^2\ox
A_\psi(\zeta_1).
$$


\begin{Lemma}
Suppose given a map $A_\psi$ satisfying \ref{apsi}\eqref{mult} and those
instances of \ref{apsi}\eqref{mreqs}, \ref{apsi}\eqref{mleqs} which involve
starting value of $\A_\psi$ on the Milnor generators $i(\zeta_1)$,
$i(\zeta_2)$, ..., where $i:\A_*\to\F_*$ is the inclusion. Then $\A_\psi$
satisfies these equations for all other values too.
\end{Lemma}

\begin{proof}

\end{proof}
\end{comment}

Now recall that, as already mentioned in \ref{L*}, according to
\cite{Baues}*{16.5} $\bar R$ is a free right $\A$-module generated by the set
$\PAR\subset\bar R$ of preadmissible relations. More explicitly, the composite
$$
R^\pre\ox\A\xto{\textrm{inclusion}\ox1}\bar R\ox\A\xto{m^\r}\bar R
$$
is an isomorphism of right $\A$-modules, where $R^\pre$ is the $\FF$-vector
space spanned by the set $\PAR$ of preadmissible relations.
Dually it follows that the composite
$$
\Phi^\r_*:\bar R_*\xto{m^\r_*}\bar R_*\ox\A_*\xto{\ro\ox1}R_\pre\ox\A_*
$$
is an isomorphism of right $\A_*$-comodules. Here $\ro:\bar R_*\onto R_\pre$ denotes
the restriction homomorphism from the space $\bar R_*$ of $\FF$-linear forms
on $\bar R$ to the space $R_\pre$ of linear forms on its subspace
$R^\pre\subset\bar R$ spanned by $\PAR$.

It thus follows that we will obtain equations equivalent to \ref{apsi}\eqref{mreqs} if
we compose both sides of these equations with the isomorphism
$1\ox\Phi^\r_*:\A_*\ox\bar R_*\to\A_*\ox R_\pre\ox\A_*$. Let us then denote
$$
(1\ox\Phi^\r_*)A_\psi(\zeta_n)=\sum_\mu\rho_{2^n-|\mu|}(\mu)\ox\mu
$$
with some unknown elements $\rho_{j}(\mu)\in(\A_*\ox R_\pre)_j$, where
$\mu$ runs through some basis of $\A_*$.

Now freedom of the right $\A_*$-comodule $\bar R_*$ on $R_\pre$ means that the
above isomorphism $\Phi^\r_*$ fits in the commutative diagram
$$
\xymatrix{
\bar R_*\ar[r]^-{\Phi^\r_*}\ar[d]^{m^\r_*}&R_\pre\ox\A_*\ar[d]^{1\ox m_*}\\
\bar R_*\ox\A_*\ar[r]^-{\Phi^\r_*\ox1}&R_\pre\ox\A_*\ox\A_*.
}
$$
It follows that we have
$$
(1\ox1\ox m_*)(1\ox\Phi^\r_*)A_\psi(\zeta_n)
=(1\ox\Phi^\r_*\ox1)(1\ox m^r_*)A_\psi(\zeta_n).
$$

Then taking into account \ref{mrC} this gives equations
$$
\sum_\mu\rho_{2^n-|\mu|}(\mu)\ox m_*(\mu)=
\sum_\mu\rho_{2^n-|\mu|}(\mu)\ox\mu\ox1+\sum_{0<k<n}(1\ox\Phi^\r_*)(C^{(n)}_{2^n-2^k+1})\ox\zeta_k,
$$
with the constants $C^{(j)}_n$ as in \ref{mrC}. This immediately determines
the elements $\rho_j(\mu)$ for $|\mu|>0$. Indeed, the above equation implies
that $(1\ox\Phi^\r_*)A_\psi(\zeta_n)$ actually lies in the subspace $\A_*\ox
R_\pre\ox\Pi\subset\A_*\ox R_\pre\ox\A_*$ where $\Pi\subset\A_*$ is the
following subspace:
$$
\Pi=\set{x\in\A_*\ \mid\ m_*(x)\in\bigoplus_{k\ge0}\A_*\ox\FF\zeta_k}.
$$
It is easy to see that actually
$$
\Pi=\bigoplus_{k\ge0}\FF\zeta_k,
$$
so we can write
$$
(1\ox\Phi^\r_*)A_\psi(\zeta_n)=\sum_{k\ge0}\rho_{2^n-2^k+1}(\zeta_k)\ox\zeta_k
$$
where we necessarily have
$$
\rho_{2^n-2^k+1}(\zeta_k)\ox1+\rho_{2^n-2^{k+1}+1}(\zeta_{k+1})\ox\zeta_1^{2^k}+\rho_{2^n-2^{j+k}+1}(\zeta_{k+2})\ox\zeta_2^{2^k}+...
=(1\ox\Phi_\r)(C^{(n)}_{2^n-2^k+1}).
$$
for all $k\ge1$. By dimension considerations, $\rho_{2^n-2^k+1}(\zeta_k)$ can only be nonzero
for $k<n$, so the number of unknowns in these equations
strictly decreases as $k$ grows. Thus moving ``backwards'' and using
successive elimination we determine all $\rho_{2^n-2^k+1}(\zeta_k)$ for $k>0$.

It is easy to compute values of the isomorphism $1\ox\Phi^\r_*$ on all elements
involved in the constants $C^{(n)}_j$. In particular, elements of the form
$\Phi^\r_*(v_j^{2^k})$ can be given by an explicit formula. One has
$$
\Phi^\r_*(v_k)=\sum_{0\le i<k}\left(\Sq^{2^k}\Sq^{2^{k-1}}\cdots\Sq^{2^{i+2}}[2^i,2^i]\right)_*\ox\zeta_i^2
$$
and
$$
\Phi^\r_*(v_k^{2^{j-1}})
=\sum_{0\le i<k}\left(\Sq^{2^{k+j-1}}\Sq^{2^{k+j-2}}\cdots\Sq^{2^{i+j+1}}[2^{i+j-1},2^{i+j-1}]\right)_*\ox\zeta_i^{2^j},
$$
so our ``upside-down'' solving gives
\begin{align*}
\rho_{2^{n-1}+1}(\zeta_{n-1})&=\zeta_1\ox[2^{n-2},2^{n-2}]_*,\\
\rho_{2^n-2^{n-2}+1}(\zeta_{n-2})&=\zeta_1^{1+2^{n-1}}\ox[2^{n-3},2^{n-3}]_*+\zeta_1\ox\left(\Sq^{2^{n-1}}[2^{n-3},2^{n-3}]\right)_*\\
\rho_{2^n-2^{n-3}+1}(\zeta_{n-3})&=\zeta_1\zeta_2^{2^{n-2}}\ox[2^{n-4},2^{n-4}]_*+\zeta_1^{1+2^{n-1}}\ox\left(\Sq^{2^{n-2}}[2^{n-4},2^{n-4}]\right)_*+\zeta_1\ox\left(\Sq^{2^{n-1}}\Sq^{2^{n-2}}[2^{n-4},2^{n-4}]\right)_*\\
\cdots\\
\rho_{2^n-2^{n-k}+1}(\zeta_{n-k})
&=\sum_{1\le i\le k}\zeta_1\zeta_{k-i}^{2^{n-k+i}}\ox\left(\Sq^{2^{n-k+i-1}}\Sq^{2^{n-k+i-2}}\cdots\Sq^{2^{n-k+1}}[2^{n-k-1},2^{n-k-1}]\right)_*
\end{align*}
for $k<n-1$.

As for $\rho_{2^n-1}(\zeta_1)$, here we do not have a general formula, but
nevertheless it is easy to compute this value explicitly. In this way we obtain, for example,
\begin{align*}
\rho_1(\zeta_1)&=0,\\
\rho_3(\zeta_1)&=0,\\
\rho_7(\zeta_1)
&
=\zeta_1^3\ox[2,2]_*
+\zeta_1^2\ox\left([3,2]_*+[2,3]_*\right),\\
\rho_{15}(\zeta_1)
&
=\zeta_1^5\zeta_2^2\ox[2,2]_*
+\zeta_1^4\zeta_2^2\ox\left([3,2]_*+[2,3]_*\right)
+\zeta_1\zeta_2^2\ox\left(\Sq^4[2,2]\right)_*
+\zeta_2^2\ox\left((\Sq^5[2,2])_*+(\Sq^4[2,3])_*\right)\\
&
+\zeta_1^5\ox\left(\Sq^6[2,2]\right)_*
+\zeta_1^4\ox\left((\Sq^7[2,2])_*+(\Sq^6[3,2])_*+(\Sq^6[2,3])_*\right),\\
\rho_{31}(\zeta_1)
&
=\zeta_1\zeta_2^4\zeta_3^2\ox[2,2]_*
+\zeta_2^4\zeta_3^2\ox\left([3,2]_*+[2,3]_*\right)
+\zeta_1^9\zeta_3^2\ox\left(\Sq^4[2,2]\right)_*\\
&
+\zeta_1^8\zeta_3^2\ox\left((\Sq^5[2,2])_*+(\Sq^4[2,3])_*\right)
+\zeta_1^9\zeta_2^4\ox\left(\Sq^6[2,2]\right)_*\\
&
+\zeta_1^8\zeta_2^4\ox\left((\Sq^7[2,2])_*+(\Sq^6[3,2])_*+(\Sq^6[2,3])_*\right)
+\zeta_1\zeta_3^2\ox\left(\Sq^8\Sq^4[2,2]\right)_*\\
&
+\zeta_3^2\ox\left((\Sq^9\Sq^4[2,2])_*+(\Sq^8\Sq^4[2,3])_*\right)
+\zeta_1\zeta_2^4\ox\left(\Sq^{10}\Sq^4[2,2]\right)_*\\
&
+\zeta_2^4\ox\left((\Sq^{11}\Sq^4[2,2])_*+(\Sq^{10}\Sq^5[2,2])_*+(\Sq^{10}\Sq^4[2,3])_*\right)
+\zeta_1^9\ox\left(\Sq^{12}\Sq^6[2,2]\right)_*\\
&
+\zeta_1^8\ox\left((\Sq^{13}\Sq^6[2,2])_*+(\Sq^{12}\Sq^6[3,2])_*+(\Sq^{12}\Sq^6[2,3])_*\right),
\end{align*}
etc.

To summarize, let us state

\begin{Proposition}\label{mrrho}
The general solution of \ref{apsi}\eqref{mreqs} for the value on $\zeta_n$ is
given by the formula
$$
A_\psi(\zeta_n)=(1\ox\Phi^\r_*)\1\sum_{k\ge0}\rho_{2^n-2^k+1}(\zeta_k)\ox\zeta_k,
$$
where the elements $\rho_j(\zeta_k)\in(\A_*\ox R_\pre)_j$ are the ones explicitly
given above for $k>0$ while $\rho_{2^n}(1)\in(\A_*\ox R_\pre)_{2^n}$ is
arbitrary.
\end{Proposition}\qed

\ 

Let us now treat the equations \ref{apsi}\eqref{mleqs} in a similar way, now using the
fact that $\bar R$ is a free \emph{left} $\A$-module on an explicit basis
$\PAR'$ (see \ref{barr} again).

Then similarly to the above dualization it follows that the
composite
$$
\Phi^\l_*:\bar R_*\xto{m^\l_*}\A_*\ox\bar R_*\xto{1\ox\ro'}\A_*\ox R'_\pre
$$
is an isomorphism of left $\A_*$-comodules, where $\ro':\bar R_*\onto
R'_\pre$ denotes the restriction homomorphism from the space $\bar R_*$ of
$\FF$-linear forms on $\bar R$ to the space $R'_\pre$ of linear forms on the
subspace ${R^\pre}'$ of $\bar R$ spanned by $\PAR'$.

Thus similarly to the above the equations \ref{apsi}\eqref{mleqs} are
equivalent to ones obtained by composing them with the isomorphism
$1\ox\Phi^\l_*:\A_*\ox\bar R_*\to\A_*\ox\A_*\ox R'_\pre$. Let us then denote
$$
(1\ox\Phi^\l_*)A_\psi(\zeta_n)=\sum_{\pi\in\PAR'}\sigma_{2^n-|\pi|}(\pi)\ox\pi_*
$$
with some unknown elements $\sigma_j(\pi)\in(\A_*\ox\A_*)_j$, where $\pi_*$
denotes the corresponding element of the dual basis, i.~e. the unique linear form on
$R'_\pre$ assigning 1 to $\pi$ and 0 to all other elements of $\PAR'$.

Now again as above, freedom of the left $\A_*$-comodule $\bar R_*$ on $R'_\pre$ means that the
above isomorphism $\Phi^\l_*$ fits in the commutative diagram
$$
\xymatrix{
\bar R_*\ar[r]^-{\Phi^\l_*}\ar[d]^{m^\l_*}&\A_*\ox R'_\pre\ar[d]^{m_*\ox1}\\
\A_*\ox\bar R_*\ar[r]^-{1\ox\Phi^\l_*}&\A_*\ox\A_*\ox R'_\pre.
}
$$
In particular one has
$$
(1\ox1\ox\Phi^\l_*)(1\ox m^\l_*)A_\psi(\zeta_n)
=(1\ox m_*\ox1)(1\ox\Phi^\l_*)A_\psi(\zeta_n).
$$
Using this, we obtain that the equations \ref{apsi}\eqref{mleqs} are
equivalent to the following system of equations
$$
(1\ox m_*-m_*\ox1)(\sigma_{2^n-|\pi|}(\pi))
=1\ox\sigma_{2^n-|\pi|}(\pi)+\varSigma_{2^n-|\pi|}(\pi),
$$
where we denote
$$
\varSigma_{2^n-|\pi|}(\pi)=\zeta_1^{2^{n-1}}\ox\sigma_{2^{n-1}-|\pi|}(\pi)+\zeta_2^{2^{n-2}}\ox\sigma_{2^{n-2}-|\pi|}(\pi)+...+\zeta_{n-2}^4\ox\sigma_{4-|\pi|}(\pi)+\zeta_{n-1}^2\ox\sigma_{2-|\pi|}(\pi).
$$

We next use the following standard fact:

\begin{Proposition}\label{contra}
For any coalgebra $C$ with the diagonal $m_*:C\to C\ox C$ and counit
$\eps:C\to\FF$ there is a contractible cochain complex of the form
$$
\xymatrix{
C\ar[r]^{d_1}
&C^{\ox2}\ar@/^/[l]^{s_1}\ar[r]^{d_2}
&C^{\ox3}\ar@/^/[l]^{s_2}\ar[r]^{d_3}
&C^{\ox4}\ar@/^/[l]^{s_3}\ar[r]^{d_4}
&\cdots,\ar@/^/[l]^{s_4}
}
$$
i.~e. one has
$$
s_nd_n+d_{n-1}s_{n-1}=1_{C^{\ox n}}
$$
for all $n$. Here,
\begin{align*}
d_1&=m_*,\\
d_2&=1\ox m_*-m_*\ox1,\\
d_3&=1\ox1\ox m_*-1\ox m_*\ox1+m_*\ox1\ox1,\\
d_4&=1\ox1\ox1\ox m_*-1\ox1\ox m_*\ox1+1\ox m_*\ox1\ox1-m_*\ox1\ox1\ox1,
\end{align*}
etc., while $s_n$ can be taken to be equal to either
$$
s_n=\eps\ox 1_{C^{\ox n}}
$$
or
$$
s_n=1_{C^{\ox n}}\ox\eps.
$$
\end{Proposition}
\qed

Now suppose given the elements
$\sigma_{2^k-|\pi|}(\pi)$, $k<n$, satisfying the equations; we must then find
$\sigma_{2^n-|\pi|}(\pi)$ with
$$
d_2\sigma_{2^n-|\pi|}(\pi)=1\ox\sigma_{2^n-|\pi|}(\pi)+\varSigma_{2^n-|\pi|}(\pi),
$$
with $\varSigma_{2^n-|\pi|}(\pi)$ as above. Then since $d_3d_2=0$, it will follow
$$
d_3(1\ox\sigma_{2^n-|\pi|}(\pi)+\varSigma_{2^n-|\pi|}(\pi))=0.
$$
Then
$$
1\ox\sigma_{2^n-|\pi|}(\pi)+\varSigma_{2^n-|\pi|}(\pi)
=(s_3d_3+d_2s_2)(1\ox\sigma_{2^n-|\pi|}(\pi)+\varSigma_{2^n-|\pi|}(\pi))
=d_2s_2(1\ox\sigma_{2^n-|\pi|}(\pi)+\varSigma_{2^n-|\pi|}(\pi))
$$
Taking here $s_n$ from the second equality of \ref{contra}, we see that one
has
$$
1\ox\sigma_{2^n-|\pi|}(\pi)
=\varSigma_{2^n-|\pi|}(\pi)+d_2\left(1\ox(1\ox\eps)(\sigma_{2^n-|\pi|}(\pi))+(1\ox1\ox\eps)(\varSigma_{2^n-|\pi|}(\pi))\right).
$$
It follows that we can reconstruct the terms $\sigma_{2^n-|\pi|}(\pi)$ from
$(1\ox\eps)\sigma_{2^n-|\pi|}(\pi)$, i.~e. from their components that lie in
$\A_*\ox\FF\subset\A_*\ox\A_*$.

Then denoting
$$
\sigma_{2^n-|\pi|}(\pi)=x_{2^n-|\pi|}(\pi)\ox1+\sigma'_{2^n-|\pi|}(\pi),
$$
with
$$
\sigma'_{2^n-|\pi|}(\pi)\in\A_*\ox\tilde\A_*,
$$
the last equation gives
$$
1\ox x_{2^n-|\pi|}(\pi)\ox1+1\ox\sigma'_{2^n-|\pi|}(\pi)
=\varSigma_{2^n-|\pi|}(\pi)+(m_*\ox1+1\ox m_*)\sum_{i\ge0}\zeta_i^{2^{n-i}}\ox
x_{2^{n-i}-|\pi|}(\pi).
$$
By collecting terms of the form $1\ox...$ on both sides, we conclude that any solution for $\sigma$ satisfies
$$
\sigma_{2^n-|\pi|}(\pi)
=m_*(x_{2^n-|\pi|}(\pi))+\sum_{i\ge0}\zeta_i^{2^{n-i}}\ox
x_{2^{n-i}-|\pi|}(\pi).
$$
Thus the equations \ref{apsi}\eqref{mleqs} are equivalent to the system of
equations
$$
(1\ox m_*+m_*\ox1)\sum_{i\ge0}\zeta_i^{2^{n-i}}\ox x_{2^{n-i}-|\pi|}(\pi)
=1\ox m_*(x_{2^n-|\pi|}(\pi))+\sum_{i\ge0}1\ox\zeta_i^{2^{n-i}}\ox x_{2^{n-i}-|\pi|}(\pi)
+\varSigma_{2^n-|\pi|}(\pi)
$$
on the elements $x_j(\pi)\in\A_j$. Substituting here back the value of
$\varSigma_{2^n-|\pi|}(\pi)$ we obtain the equations
\begin{multline*}
\sum_{i\ge0}\zeta_i^{2^{n-i}}\ox m_*(x_{2^{n-i}-|\pi|}(\pi))
+\sum_{i\ge0}m_*(\zeta_i)^{2^{n-i}}\ox x_{2^{n-i}-|\pi|}(\pi)
=1\ox m_*(x_{2^n-|\pi|}(\pi))+\sum_{i\ge0}1\ox\zeta_i^{2^{n-i}}\ox
x_{2^{n-i}-|\pi|}(\pi)\\
+\sum_{i>0}\zeta_i^{2^{n-i}}\ox m_*(x_{2^{n-i}-|\pi|}(\pi))
+\sum_{i'>0,j\ge0}\zeta_{i'}^{2^{n-i'}}\ox\zeta_j^{2^{n-i'-j}}\ox x_{2^{n-i'-j}-|\pi|}(\pi).
\end{multline*}
These equations easily reduce to
$$
m_*(\zeta_i)^{2^{n-i}}=1\ox\zeta_i^{2^{n-i}}+\sum_{0\le
j<i}\zeta_{i-j}^{2^{n-(i-j)}}\ox\zeta_j^{2^{n-i}},
$$
which is identically true. We thus conclude

\begin{Proposition}\label{mlx}
The general solution $A_\psi(\zeta_n)$ of \ref{apsi}\eqref{mleqs} is determined by
$$
A_\psi(\zeta_n)=(1\ox\Phi^\l_*)\1\sum_{\pi\in\PAR'}\left(x_{2^n-|\pi|}(\pi)\ox1+\tilde
m_*(x_{2^n-|\pi|}(\pi))+\sum_{i>0}\zeta_i^{2^{n-i}}\ox
x_{2^{n-i}-|\pi|}(\pi)\right)\ox\pi_*,
$$
where $x_j(\pi)\in\A_j$ are arbitrary homogeneous elements.
\end{Proposition}\qed

Now to put together \ref{mrrho} and \ref{mlx} we must use the dual
$$
\Phi_*:R_\pre\ox\A_*\to\A_*\ox R'_\pre
$$
of the composite isomorphism
$$
\Phi:\A\ox{R^\pre}'\xto{{\Phi^\l}\1}\bar R\xto{\Phi^\r}R^\pre\ox\A.
$$

We will need

\begin{Lemma}
There is an inclusion
$$
\Phi_*\left(R_\pre\ox\FF1\right)\subset\A_*\ox{R'_\pre}^{\le2},
$$
where
$$
{R'_\pre}^{\le2}\subset R'_\pre
$$
is the subspace of those linear forms on ${R^\pre}'$ which vanish on all left
preadmissible elements $[n,m]a\in\PAR'$ with $a\in\tilde\A$.

Similarly, there is an inclusion
$$
\Phi_*\1\left(\FF1\ox R'_\pre\right)\subset{R_\pre}^{\le2}\ox\A_*,
$$
where
$$
{R_\pre}^{\le2}\subset R_\pre
$$
is the subspace of those linear forms on $R^\pre$ which vanish on all right
preadmissible elements $a[n,m]$ with $a\in\tilde\A$.
\end{Lemma}

\begin{proof}
Dualizing, what we have to prove for the first inclusion is that given any
admissible monomial $a\in\A$ and any $[n,m]b\in\PAR'$ with $b\in\tilde\A$, in
$\bar R$ one has the equality
$$
a[n,m]b=\sum_ia_i[n_i,m_i]b_i
$$
with $a_i[n_i,m_i]\in\PAR$ and admissible monomials $b_i\in\tilde\A$. Indeed,
considering $a$ as a monomial in $\F_0$ there is a unique way to write
$$
a[n,m]=\sum_ia_i[n_i,m_i]c_i
$$
in $\F_0$, with $a_i[n_i,m_i]\in\PAR$ and $c_i$ some (not necessarily
admissible or belonging to $\tilde\F_0$) monomials in the $\Sq^k$ generators
of $\F_0$. Thus in $\F_0$ we have
$$
a[n,m]b=\sum_ia_i[n_i,m_i]c_ib.
$$
In $\bar R$ we may replace each $c_ib$ with a sum of admissible monomials of
the same degree; obviously this degree is positive as $b\in\tilde\A$.

The proof for the second inclusion is exactly similar.
\end{proof}

This lemma implies that for any simultaneous solution $A_\psi(\zeta_n)$ of
\ref{apsi}\eqref{mreqs} and \ref{apsi}\eqref{mleqs}, the elements in $\A_*\ox
R_\pre\ox\A_*$ and $\A_*\ox\A_*\ox R'_\pre$ corresponding to it according to,
respectively, \ref{mrrho} and \ref{mlx}, satisfy
\begin{multline*}
\sum_{\substack{a\in\tilde\A\\{}[k,l]a\in\PAR'}}\left(x_{2^n-k-l-|a|}([k,l]a)\ox1+\tilde
m_*(x_{2^n-k-l-|a|}([k,l]a))+\sum_{i>0}\zeta_i^{2^{n-i}}\ox
x_{2^{n-i}-k-l-|a|}([k,l]a)\right)\ox([k,l]a)_*\\
=(1\ox1\ox\varrho^{>2})(1\ox\Phi_*)\left(\sum_{k>0}\rho_{2^n-2^k+1}(\zeta_k)\ox\zeta_k\right),
\end{multline*}
where
$$
\varrho^{>2}:R_\pre'\onto{R_\pre'}^{>2}
$$
is the restriction of linear forms on ${R^\pre}'$ to the subspace spanned by
the subset of $\PAR'$ consisting of the left preadmissible relations of the
form $[k,l]a$ with $a\in\tilde\A$. Indeed the remaining part of the element
from \ref{mrrho} is
$$
\rho_{2^n}(1)\ox1,
$$
and according to the lemma its image under $1\ox\Phi_*$ goes to zero under the
map $\varrho^{>2}$.

Since the elements $\rho_{2^n-2^k+1}(\zeta_k)$ are explicitly given for all $k>0$, this
allows us to explicitly determine all elements $x_j([k,l]a)$ for
$[k,l]a\in\PAR'$ with $a\in\tilde\A$. For example, in low degrees we obtain
\begin{align*}
x_2([2,3]\Sq^1)=x_2([3,2]\Sq^1)&=\zeta_1^2,\\
x_3([2,2]\Sq^1)&=\zeta_1^3,\\
x_{10}([2,3]\Sq^1)=x_{10}([3,2]\Sq^1)&=\zeta_1^4\zeta_2^2,\\
x_{11}([2,2]\Sq^1)&=\zeta_1^5\zeta_2^2,\\
x_{26}([2,3]\Sq^1)=x_{26}([3,2]\Sq^1)&=\zeta_2^4\zeta_3^2,\\
x_{27}([2,2]\Sq^1)&=\zeta_1\zeta_2^4\zeta_3^2,
\end{align*}
with all other $x_j([k,l]a)=0$ for $j<32$ and $[k,l]a\in\PAR'$ with
$a\in\tilde\A$.

It remains to deal with  the elements $x_j([k,l])$. These shall satisfy
\begin{multline*}
\sum_{k<2l}\left(x_{2^n-k-l}([k,l])\ox1+\tilde
m_*(x_{2^n-k-l}([k,l]))+\sum_{i>0}\zeta_i^{2^{n-i}}\ox
x_{2^{n-i}-k-l}([k,l])\right)\ox[k,l]_*\\
=(1\ox\Phi_*)\left(\rho_{2^n}(1)\ox1\right)+(1\ox1\ox\varrho^{\le2})(1\ox\Phi_*)\left(\sum_{k>0}\rho_{2^n-2^k+1}(\zeta_k)\ox\zeta_k\right),
\end{multline*}
where now
$$
\varrho^{\le2}:R_\pre'\onto{R_\pre'}^{\le2}
$$
is the restriction of linear forms on ${R^\pre}'$ to the subspace spanned by
the Adem relations. The last summand
$D_n=(1\ox1\ox\varrho^{\le2})(1\ox\Phi_*)\left(\sum_{k>0}\rho_{2^n-2^k+1}(\zeta_k)\ox\zeta_k\right)$
is again explicitly given; for example, in low degrees it is equal to
\begin{align*}
D_1&=0,\\
D_2&=0,\\
D_3&=\left(\zeta_1\ox\zeta_1\right)^2\ox[2,2]_*,\\
D_4&=\left(\zeta_1^2\zeta_2\ox\zeta_1+\zeta_2\ox\zeta_2+\zeta_1^2\ox\zeta_1\zeta_2\right)^2\ox[2,2]_*,\\
D_5&=\left(
 \zeta_2^2\zeta_3\ox\zeta_1
+\zeta_1^4\zeta_3\ox\zeta_2
+\zeta_1^4\zeta_2^2\ox\zeta_1\zeta_2
+\zeta_1^4\ox\zeta_2\zeta_3
+\zeta_3\ox\zeta_3
+\zeta_2^2\ox\zeta_1\zeta_3
\right)^2\ox[2,2]_*.
\end{align*}
Then finally the equations that remain to be solved can be equivalently
written as follows:
\begin{multline*}
(1\ox1\ox\tilde\eps)(1\ox\Phi_*)\1\left(\sum_{k<2l}\left(x_{2^n-k-l}([k,l])\ox1+\tilde
m_*(x_{2^n-k-l}([k,l]))+\sum_{i>0}\zeta_i^{2^{n-i}}\ox
x_{2^{n-i}-k-l}([k,l])\right)\ox[k,l]_*\right)\\
=(1\ox1\ox\tilde\eps)(1\ox\Phi_*)\1(D_n),
\end{multline*}
where
$$
\tilde\eps:\A_*\onto\tilde\A_*
$$
is the projection to the positive degree part, i.~e. maps 1 to 0 and all
homogeneous positive degree elements to themselves. Again, the right hand
sides of these equations are explicitly given constants, for example, in low
degrees they are given by

\begin{tabular}{cl}
$0$,&$n=1$;\\
$0$,&$n=2$;\\
$\zeta_1^2\ox[2,2]_*\ox\zeta_1^2$,&$n=3$;\\
$\left(\zeta_1^4\zeta_2^2\ox[2,2]_*+\zeta_2^2\ox(\Sq^4[2,2])_*+\zeta_1^4\ox(\Sq^6[2,2])_*\right)\ox\zeta_1^2$,&$n=4$;\\
$\left(\zeta_2^4\zeta_3^2\ox[2,2]_*+\zeta_1^8\zeta_3^2\ox(\Sq^4[2,2])_*+\zeta_1^8\zeta_2^4\ox(\Sq^6[2,2])_*+\zeta_3^2\ox(\Sq^8\Sq^4[2,2])_*\right.$\\
$\left.+\zeta_2^4\ox(\Sq^{10}\Sq^4[2,2])_*+\zeta_1^8\ox(\Sq^{12}\Sq^6[2,2])_*\right)\ox\zeta_1^2$,&$n=5$.
\end{tabular}

\ 

\ 

\ 

One possible set of solutions for $\zeta_k$ with $k\le4$ is given by
\begin{align*}
x_6([1,1])&=\zeta_1^6+\zeta_2^2,\\
x_8([2,6])&=\zeta_1^8,\\
x_{12}([1,3])&=\zeta_2^4,\\
x_{13}([1,2])&=\zeta_2^2\zeta_3,\\
x_{24}([2,6])&=\zeta_2^8,\\
x_{28}([1,3])&=\zeta_3^4,\\
x_{29}([1,2])&=\zeta_3^2\zeta_4
\end{align*}
and all remaining $x_j([k,l])=0$ for $j+k+l\le32$.

\ 

Or equivalently one might give the same solution ``on the other side of $\Phi$'' by
\begin{align*}
\rho_2(1)&=0,\\
\rho_4(1)&=0,\\
\rho_8(1)&=\zeta_1^2\ox(\Sq^4[1,1])_*+\left(\zeta_1^6+\zeta_2^2\right)\ox[1,1]_*,\\
\rho_{16}(1)&
=\zeta_1^4\ox\left(\Sq^6\Sq^3[1,2]\right)_*
+\zeta_2^2\ox\left(\Sq^5\Sq^2[1,2]\right)_*
+\zeta_3\ox\left(\Sq^4\Sq^2[1,2]\right)_*\\
&
+\zeta_1^8\ox\left((\Sq^6[1,1])_*+(\Sq^4[1,3])_*+[2,6]_*\right)
+\zeta_1^4\zeta_2^2\ox\left(\Sq^3[1,2]\right)_*
+\zeta_1^4\zeta_3\ox\left(\Sq^2[1,2]\right)_*\\
&
+\zeta_2^4\ox[1,3]_*
+\zeta_2^2\zeta_3\ox[1,2]_*,\\
\rho_{32}(1)&
=\zeta_1^8\ox\left(\Sq^{12}\Sq^6\Sq^3[1,2]\right)_*
+\zeta_2^4\ox\left(\Sq^{10}\Sq^5\Sq^2[1,2]\right)_*
+\zeta_3^2\ox\left(\Sq^9\Sq^4\Sq^2[1,2]\right)_*\\
&
+\zeta_4\ox\left(\Sq^8\Sq^4\Sq^2[1,2]\right)_*
+\zeta_1^8\zeta_2^4\ox\left(\Sq^6\Sq^3[1,2]\right)_*
+\zeta_1^8\zeta_3^2\ox\left(\Sq^5\Sq^2[1,2]\right)_*
+\zeta_1^8\zeta_4\ox\left(\Sq^4\Sq^2[1,2]\right)_*\\
&
+\zeta_2^8\ox\left((\Sq^4[1,3])_*+(\Sq^6[1,1])_*+[2,6]_*\right)
+\zeta_2^4\zeta_3^2\ox\left(\Sq^3[1,2]\right)_*
+\zeta_2^4\zeta_4\ox\left(\Sq^2[1,2]\right)_*\\
&
+\zeta_3^4\ox[1,3]_*
+\zeta_3^2\zeta_4\ox[1,2]_*.
\end{align*}

This then gives the solution itself as follows:

\ 

\begin{align*}
A_\psi(\zeta_1)&=0,\\
\\
A_\psi(\zeta_2)&=0,\\
\\
A_\psi(\zeta_3)
&
=\zeta_1\ox M_{2221}
+\zeta_1^2\ox\left(M_{411}+M_{231}+M_{2121}+\zeta_1M_{221}+\zeta_1^2M_{11}^2+M_3^2\right)
+\zeta_1^3\ox M_{221}\\
&
+\left(\zeta_1^6+\zeta_2^2\right)\ox M_{11},\\
\\
A_\psi(\zeta_4)
=\zeta_1&\ox\left(M_{82221}+M_{44421}+M_{424221}+M_{46221}\right)\\
+\zeta_1^4&\ox\left(\zeta_1^4\zeta_2M_5+\zeta_1^4M_{211}^2+\zeta_1^2M_{2111}^2+M_{4521}+M_{23421}+M_{62121}+M_{6231}+M_{2721}+M_{41421}+M_{44121}\right.\\
&
+M_{651}+M_{4431}+M_{24231}+M_{242121}+M_{2451}+M_{831}+M_{8121}+\zeta_1^2\zeta_3M_3+\zeta_2^3M_3+\zeta_1^6M_3^2+\zeta_1^2M_5^2\\
&
+\zeta_2M_{2421}+\zeta_1^2M_{41}^2+\zeta_2M_{54}+\zeta_3M_{32}+\zeta_2M_{621}+\zeta_2M_9+\zeta_2M_{441}+\zeta_2M_{342}+\zeta_3M_{41}\\
&
\left.+\zeta_2M_{72}+\zeta_3M_5+\zeta_2M_{432}+\zeta_1^2M_{32}^2+M_{6321}+\zeta_1M_{6221}+\zeta_1M_{4421}+\zeta_1M_{24221}+M_{24321}\right)\\
+\zeta_1^5&\ox\left(M_{24221}+M_{6221}+M_{4421}\right)\\
+\zeta_2^2&\ox\left(M_{4231}+M_{42121}+M_{41}^2+M_5^2+M_{2111}^2+M_{32}^2+M_{721}+M_{3421}+M_{451}+\zeta_1\zeta_2^2M_3+\zeta_1M_{54}+\zeta_1^5M_5\right.\\
&
\left.+\zeta_1^4M_3^2+\zeta_1M_{72}+\zeta_1M_{2421}+\zeta_3M_3+\zeta_1M_{441}+\zeta_1M_9+\zeta_1M_{621}+\zeta_1M_{342}+\zeta_1M_{432}+\zeta_1M_{4221}+M_{4321}\right)\\
+\zeta_3&\ox\left(M_{54}+M_{2421}+M_{342}+M_{441}+M_{72}+M_{621}+M_9+M_{432}+\zeta_2^2M_3+\zeta_1^4M_5\right)\\
+\zeta_1\zeta_2^2&\ox M_{4221}\\
+\zeta_1^8&\ox\left(M_{211}^2+\zeta_2M_5+M_{4121}+M_{31}^2+M_{2411}+M_{251}+M_{611}+\zeta_2M_{32}+\zeta_1^2\zeta_2M_3+\zeta_1^2M_3^2+M_{2321}+\zeta_2M_{41}\right)\\
+\zeta_1^9&\ox M_{2221}\\
+\zeta_1^4\zeta_2^2&\ox\left(M_{231}+M_{2121}+M_{51}+\zeta_1^2M_{11}^2+\zeta_1M_{221}+\zeta_1M_{41}+\zeta_1M_5+\zeta_1^3M_3+M_{321}+\zeta_1M_{32}+\zeta_2M_3\right)\\
+\zeta_1^5\zeta_2^2&\ox M_{221}\\
+\zeta_1^4\zeta_3&\ox\left(M_5+M_{41}+M_{32}+\zeta_1^2M_3\right)\\
+\zeta_2^4&\ox\left(M_{31}+\zeta_1M_3\right)\\
+\zeta_2^2\zeta_3&\ox M_3,
\end{align*}
\begin{align*}
A_\psi(\zeta_5)
=\zeta_1&\ox\left(M_{8484421}+M_{888421}+M_{\underline{16}82221}+M_{\underline{16}424221}+M_{\underline{16}44421}+M_{8\underline{12}4421}+M_{8\underline{12}6221}\right.\\
&
\left.+M_{8\underline{12}24221}+M_{\underline{16}46221}+M_{84\underline{10}4221}+M_{8486221}+M_{84824221}+M_{84284221}\right)\\
+\zeta_1^8&\ox\left(M_{431211}^2+M_{422211}^2+M_{2721}^2+M_{421221}^2+M_{34221}^2+M_{7221}^2+M_{41421}^2+M_{43221}^2\right.\\
&
+M_{\underline{12}24321}+M_{32}^2\zeta_3^2+M_{54}\zeta_4+\zeta_1M_{88421}+M_{4284321}+\zeta_2^2M_{2421}^2\\
&
+\zeta_1M_{\underline{12}24221}+M_{3842}\zeta_3+M_{342}\zeta_4+M_{8426121}+M_{8441}\zeta_3+M_{4\underline{10}4321}+M_{\underline{12}6321}\\
&
+\zeta_1M_{\underline{12}4421}+M_{41}^4\zeta_1^4+M_{41}^2\zeta_3^2+\zeta_1M_{484421}+M_{243111}^2+\zeta_2^2M_{432}^2+\zeta_3M_{\underline{11}42}\\
&
+\zeta_2^2M_{342}^2+M_{441}\zeta_4+M_3^8+\zeta_2^4M_3^4+M_{321}^4+M_{2451}^2+M_{35211}^2+M_{51}^4+M_{411}^4+\zeta_3M_{584}\\
&
+M_{831}^2+M_{8121}^2+M_{621}\zeta_4+M_{651}^2+M_{23421}^2+\zeta_2^2M_{621}^2+\zeta_3M_{98}+\zeta_3M_{8342}+M_{242211}^2\\
&
+M_{24411}^2+M_{7311}^2+M_{486321}+M_{2412111}^2+M_{34311}^2+M_{4824321}+M_{252111}^2+M_{86631}\\
&
+M_{8624121}+M_{8444121}+M_{844431}+M_{844521}+M_{48831}+M_{862431}+M_{866121}\\
&
+M_{8441421}+M_{8423421}+M_{84212421}+M_{4862121}+M_{4823421}+M_{4284231}\\
&
+M_{4824231}+M_{48242121}+M_{\underline{12}62121}+M_{\underline{12}4431}+M_{\underline{12}4521}+M_{\underline{12}44121}+M_{\underline{12}41421}+M_{4844121}\\
&
+M_{4841421}+M_{48651}+M_{\underline{12}6231}+M_{\underline{12}2451}+M_{4\underline{10}451}+M_{\underline{12}2721}+M_{4\underline{10}42121}+M_{\underline{12}242121}\\
&
+M_{484521}+M_{4\underline{10}721}+M_{\underline{12}651}+M_{486231}+M_{482451}+M_{482721}+M_{\underline{12}24231}+M_{4\underline{10}4231}+M_{428451}\\
&
+M_{428721}+M_{\underline{12}23421}+M_{4\underline{10}3421}+M_{42\underline{11}421}+M_{42842121}+M_{\underline{14}2521}+M_{6\underline{10}521}+M_{\underline{14}24121}\\
&
+M_{6\underline{10}4121}+M_{628521}+M_{\underline{14}21421}+M_{629421}+M_{6\underline{10}1421}+M_{68631}+M_{682431}+M_{686121}+M_{682521}\\
&
+M_{628431}+M_{6824121}+M_{6821421}+M_{6284121}+M_{6281421}+M_{6218421}+M_{4\underline{12}431}+M_{\underline{12}8121}+M_{4\underline{12}521}\\
&
+M_{\underline{12}831}+M_{448431}+M_{4\underline{12}4121}+M_{448521}+M_{4\underline{12}1421}+M_{449421}+M_{4484121}+M_{4481421}+M_{4418421}\\
&
+M_{\underline{14}2431}+M_{6\underline{10}431}+M_{\underline{14}6121}+M_{\underline{14}631}+M_{341211}^2+M_{8621}\zeta_3+M_{6321}^2+\zeta_1^{12}M_3^4+\zeta_3^3M_3\\
&
+\zeta_3M_{\underline{13}4}+M_{72}\zeta_4+\zeta_2^2M_{72}^2+M_{842631}+M_{421311}^2+M_{314211}^2+M_{26211}^2+M_{6411}^2+\zeta_3M_{82421}\\
&
+\zeta_1^4M_5^4+M_{224211}^2+M_9\zeta_4+M_{43311}^2+M_{24321}^2+M_{62211}^2+M_{612111}^2+\zeta_1^4M_{32}^4+M_{63111}^2\\
&
+\zeta_3M_{854}+\zeta_3M_{8432}+\zeta_3M_{\underline{10}421}+\zeta_2^2M_{441}^2+\zeta_3M_{28421}+\zeta_2^4\zeta_3M_5+\zeta_1^8\zeta_2^2M_5^2+M_{484431}\\
&
+\zeta_1^4\zeta_4M_5+\zeta_1^4M_3^2\zeta_3^2+M_3^2\zeta_2^6+M_3\zeta_4\zeta_2^2+M_9\zeta_3\zeta_1^8+\zeta_3^2M_5^2+M_{71211}^2+M_{4238421}\\
&
+\zeta_1M_{4284221}+\zeta_1M_{4\underline{10}4221}+\zeta_1M_{486221}+\zeta_2^2M_9^2+\zeta_4M_{432}+\zeta_2^2M_{54}^2+\zeta_3M_{872}+M_{4283421}\\
&
\left.+M_{862521}+M_{488121}+M_{8621421}+\zeta_3M_{\underline{17}}+M_{2142111}^2+\zeta_1M_{\underline{12}6221}+\zeta_1M_{4824221}\right)\\
+\zeta_1^9&\ox\left(M_{4\underline{10}4221}+M_{4824221}+M_{88421}+M_{\underline{12}6221}+M_{4284221}+M_{484421}+M_{\underline{12}4421}+M_{486221}+M_{\underline{12}24221}\right)\\
+\zeta_2^4&\ox\left(M_{283421}+M_{2\underline{11}421}+M_{\underline{12}521}+M_{8831}+M_{88121}+M_{\underline{10}42121}+M_{862121}+M_{82451}+M_{82721}+M_{823421}\right.\\
&
+M_{284231}+M_{86231}+M_{824231}+M_{844121}+M_{841421}+M_{28451}+M_{\underline{10}4231}+M_{8651}+M_{\underline{10}451}+M_{84521}\\
&
+M_{84431}+M_{2842121}+M_{8242121}+M_{\underline{12}431}+M_{484121}+M_{418421}+M_{\underline{12}4121}+M_{48431}+M_{28721}+\zeta_2M_{98}\\
&
+M_{\underline{10}3421}+M_{\underline{10}721}+\zeta_1^8\zeta_2M_9+\zeta_1^2\zeta_2^4M_3^2+\zeta_2\zeta_3^2M_3+\zeta_1^2\zeta_4M_3+M_{238421}+M_{48521}+M_{49421}+M_{\underline{12}1421}\\
&
+M_{481421}+\zeta_2M_{8342}+M_{86321}+\zeta_1M_{284221}+\zeta_1M_{86221}+\zeta_1M_{84421}+\zeta_1M_{824221}+\zeta_1M_{\underline{10}4221}+M_{824321}\\
&
+\zeta_2M_{8432}+\zeta_2M_{\underline{11}42}+\zeta_2M_{872}+\zeta_2M_{28421}+\zeta_2M_{8441}+\zeta_2M_{3842}+\zeta_1^2M_{72}^2+\zeta_1^2M_{621}^2+\zeta_4M_{41}+\zeta_2M_{584}\\
&
+M_{2421}^2\zeta_1^2+\zeta_1^2M_{432}^2+M_{32}\zeta_4+M_{54}^2\zeta_1^2+\zeta_2M_{\underline{10}421}+\zeta_1^2M_{342}^2+\zeta_1^2M_{441}^2+\zeta_2M_{\underline{13}4}+\zeta_2M_{82421}+\zeta_2M_{854}\\
&
\left.+\zeta_2M_{8621}+\zeta_2^5M_5+\zeta_1^{10}M_5^2+\zeta_2M_{\underline{17}}+M_5\zeta_4+M_9^2\zeta_1^2+\zeta_1^2M_{42111}^2+M_{\underline{10}4321}+M_{4211}^2\zeta_1^4+M_{284321}\right)\\
+\zeta_1\zeta_2^4&\ox\left(M_{86221}+M_{284221}+M_{\underline{10}4221}+M_{84421}+M_{824221}\right)\\
+\zeta_3^2&\ox\left(M_{84231}+M_{2421}^2+M_{342}^2+M_{441}^2+M_{72}^2+M_{54}^2+M_{621}^2+M_9^2+M_{432}^2+M_{42111}^2+M_{842121}+M_{8451}\right.\\
&
+M_{\underline{11}421}+M_{8721}+M_{38421}+M_{83421}+M_{84321}+M_5^2\zeta_1^8+M_3\zeta_4+M_3^2\zeta_2^4+\zeta_1^9M_9+\zeta_1M_{\underline{17}}+\zeta_1M_{98}\\
&
+\zeta_1M_{\underline{13}4}+\zeta_1M_{854}+\zeta_1M_{584}+\zeta_1M_{8441}+\zeta_1M_{\underline{11}42}+\zeta_1M_{872}+\zeta_1M_{8342}+\zeta_1M_{8432}+\zeta_1M_{3842}\\
&
\left.+\zeta_1M_{28421}+\zeta_1M_{\underline{10}421}+\zeta_1M_{82421}+\zeta_1M_{8621}+\zeta_1M_{84221}+\zeta_1M_3\zeta_3^2+\zeta_1M_5\zeta_2^4\right)\\
+\zeta_1\zeta_3^2&\ox M_{84221}\\
+\zeta_4&\ox\left(M_{584}+M_{854}+M_{\underline{13}4}+M_{872}+M_{8432}+M_{28421}+M_{98}+M_{\underline{17}}+M_{8342}+M_{\underline{11}42}+M_{8441}+M_{8621}\right.\\
&
\left.+M_{\underline{10}421}+M_{3842}+M_{82421}+\zeta_1^8M_9+\zeta_2^4M_5+\zeta_3^2M_3\right)\\
+\zeta_1^{17}&\ox\left(M_{82221}+M_{44421}+M_{424221}+M_{46221}\right)
\end{align*}
\begin{align*}
+\zeta_1^8\zeta_2^4&\ox\left(\zeta_1^4\zeta_2M_5+\zeta_1^4M_{211}^2+\zeta_1^2M_{2111}^2+M_{4521}+M_{23421}+M_{62121}+M_{6231}+M_{2721}+M_{41421}+M_{44121}+M_{651}\right.\\
&
+M_{4431}+M_{24231}+M_{242121}+M_{2451}+M_{831}+M_{8121}+M_3\zeta_3\zeta_1^2+\zeta_2^3M_3+\zeta_1^6M_3^2+\zeta_1^2M_5^2+\zeta_2M_{2421}+\zeta_1^2M_{41}^2\\
&
+\zeta_2M_{54}+\zeta_3M_{32}+\zeta_2M_{621}+\zeta_2M_9+\zeta_2M_{441}+\zeta_2M_{342}+\zeta_3M_{41}+\zeta_2M_{72}+\zeta_3M_5+\zeta_2M_{432}+\zeta_1^2M_{32}^2+M_{6321}\\
&
\left.+\zeta_1M_{6221}+\zeta_1M_{4421}+\zeta_1M_{24221}+M_{24321}\right)\\
+\zeta_1^9\zeta_2^4&\ox\left(M_{24221}+M_{6221}+M_{4421}\right)\\
+\zeta_1^8\zeta_3^2&\ox\left(M_{4231}+M_{42121}+M_{41}^2+M_5^2+M_{2111}^2+M_{32}^2+M_{721}+M_{3421}+M_{451}+\zeta_1\zeta_2^2M_3+\zeta_1M_{54}+\zeta_1^5M_5+\zeta_1^4M_3^2\right.\\
&
\left.+\zeta_1M_{72}+M_{2421}\zeta_1+M_3\zeta_3+\zeta_1M_{441}+\zeta_1M_9+\zeta_1M_{621}+\zeta_1M_{342}+\zeta_1M_{432}+\zeta_1M_{4221}+M_{4321}\right)\\
+\zeta_1^8\zeta_4&\ox\left(M_{54}+M_{2421}+M_{342}+M_{441}+M_{72}+M_{621}+M_9+M_{432}+M_3\zeta_2^2+M_5\zeta_1^4\right)\\
+\zeta_1^9\zeta_3^2&\ox M_{4221}\\
+\zeta_2^8&\ox\left(M_{211}^2+\zeta_2M_5+M_{4121}+M_{31}^2+M_{2411}+M_{251}+M_{611}+\zeta_2M_{32}+\zeta_2M_3\zeta_1^2+\zeta_1^2M_3^2+M_{2321}+\zeta_2M_{41}\right)\\
+\zeta_1\zeta_2^8&\ox M_{2221}\\
+\zeta_2^4\zeta_3^2&\ox\left(M_{231}+M_{2121}+M_{51}+\zeta_1^2M_{11}^2+\zeta_1M_{221}+\zeta_1M_{41}+\zeta_1M_5+\zeta_1^3M_3+M_{321}+\zeta_1M_{32}+\zeta_2M_3\right)\\
+\zeta_2^4\zeta_4&\ox\left(M_5+M_{41}+M_{32}+\zeta_1^2M_3\right)\\
+\zeta_1\zeta_2^4\zeta_3^2&\ox M_{221}\\
+\zeta_3^4&\ox\left(M_{31}+\zeta_1M_3\right)\\
+\zeta_3^2\zeta_4&\ox M_3
\end{align*}



\chapter*{}

This solution satisfies
$A_\psi(\zeta_k)=0$ for $k<3$,
\begin{align*}
(1\ox\Phi_\l)(A_\psi(\zeta_3))
&
=\left(\zeta_2\ox1+\zeta_1^2\ox\zeta_1\right)\ox[2,3]_*\\
&+\left(\zeta_1^3\ox1+\zeta_1^2\ox\zeta_1+\zeta_1\ox\zeta_1^2\right)\ox([2,2]\Sq^1)_*\\
&+\zeta_1^2\ox1\ox[3,3]_*\\
&+\zeta_1^2\ox1\ox\left(([3,2]\Sq^1)_*+([2,3]\Sq^1)_*\right),\\
\\
(1\ox\Phi_\r)(A_\psi(\zeta_3))
&
=\zeta_2\ox[2,3]_*\ox1\\
&
+\zeta_1^2\ox[3,3]_*\ox1\\
&
+\zeta_1^2\ox\left([2,3]_*+[3,2]_*\right)\ox\zeta_1\\
&
+\zeta_1\ox[2,2]_*\ox\zeta_2,
\end{align*}
and
\begin{align*}
(1\ox\Phi_\l)(A_\psi(\zeta_4))
&
=\left(
 \zeta_1^4\zeta_3\ox1
+\zeta_1^4\zeta_2^2\ox\zeta_1
+\zeta_1^8\ox\zeta_2
+\zeta_2^2\ox\zeta_1^5
+\zeta_1^4\ox\zeta_1^4\zeta_2
+\zeta_1^4\ox\zeta_3
+\zeta_3\ox\zeta_1^4\right)\ox[2,3]_*\\
&
+\left(
 \zeta_1^5\zeta_2^2\ox1
+\zeta_1^4\zeta_2^2\ox\zeta_1
+\zeta_1^9\ox\zeta_1^2
+\zeta_1^8\ox\zeta_1^3
+\zeta_1\zeta_2^2\ox\zeta_1^4
+\zeta_2^2\ox\zeta_1^5
+\zeta_1^5\ox\zeta_1^6
+\zeta_1^5\ox\zeta_2^2\right.\\
&
 \left.\ \ 
+\zeta_1^4\ox\zeta_1^7
+\zeta_1^4\ox\zeta_1\zeta_2^2
+\zeta_1\ox\zeta_1^4\zeta_2^2\right)\ox([2,2]\Sq^1)_*\\
&
+\left(
 \zeta_1^4\zeta_2^2\ox1
+\zeta_1^8\ox\zeta_1^2
+\zeta_1^4\ox\zeta_2^2
+\zeta_2^2\ox\zeta_1^4
+\zeta_1^4\ox\zeta_1^6\right)\ox[3,3]_*\\
&
+\left(
 \zeta_1^4\zeta_2^2\ox1
+\zeta_1^8\ox\zeta_1^2
+\zeta_1^4\ox\zeta_2^2
+\zeta_2^2\ox\zeta_1^4
+\zeta_1^4\ox\zeta_1^6\right)\ox\left(([3,2]\Sq^1)_*+([2,3]\Sq^1)_*\right),\\
\\
(1\ox\Phi_\r)(A_\psi(\zeta_4))
&
=\left(\zeta_1^4\ox(\Sq^6[3,3])_*
+\zeta_2^2\ox(\Sq^5[2,3])_*
+\zeta_3\ox(\Sq^4[2,3])_*
+\zeta_1^4\zeta_2^2\ox[3,3]_*\right.\\
&
\ \ \left.+\zeta_1^4\zeta_3\ox[2,3]_*\right)\ox1\\
&
+\left(\zeta_1^4\ox(\Sq^7[2,2])_*
+\zeta_1^4\ox(\Sq^6[2,3])_*
+\zeta_1^4\ox(\Sq^6[3,2])_*
+\zeta_1^5\ox(\Sq^6[2,2])_*\right.\\
&
\ \ +\zeta_2^2\ox(\Sq^5[2,2])_*
+\zeta_2^2\ox(\Sq^4[2,3])_*
+\zeta_1\zeta_2^2\ox(\Sq^4[2,2])_*
+\zeta_1^4\zeta_2^2\ox[2,3]_*\\
&
\ \ \left.+\zeta_1^4\zeta_2^2\ox[3,2]_*
+\zeta_1^5\zeta_2^2\ox[2,2]_*\right)\ox\zeta_1\\
&
+\left(\zeta_1\ox(\Sq^8[2,2])_*
+\zeta_1^8\ox[3,2]_*
+\zeta_1^9\ox[2,2]_*\right)\ox\zeta_2\\
&
+\zeta_1^8\ox[2,3]_*\ox\zeta_1^3\\
&
+\zeta_1^8\ox[2,2]_*\ox\zeta_1\zeta_2\\
&
+\zeta_1\ox[4,4]_*\ox\zeta_3.
\end{align*}

The solutions themselves are readily obtained from these. For example, one has
\begin{align*}
A_\psi(\zeta_3)
&
=\zeta_1\ox\left(\zeta_1^3M_{11}^2
+\zeta_1^2M_{11}M_3
+\zeta_1M_{2211}
+\zeta_2M_{31}
+\zeta_2M_{11}^2
+M_{11}M_{32}
+\zeta_1^3M_{1111}\right.\\
&
+\zeta_2M_{1111}
+\zeta_1M_{321}
+\zeta_1\zeta_2M_3
+M_{2221}
+\zeta_1^2M_{311}
+\zeta_1M_{11}M_{31}
+M_{3121}\\
&\left.
+\zeta_1^2M_{221}
+\zeta_1M_{11}M_{211}
+\zeta_1M_{3111}\right)\\
&
+\zeta_1^2\ox\left(
M_{411}
+M_{231}
+M_{51}
+\zeta_1M_{41}
+\zeta_1M_{5}
+\zeta_1^2M_{31}
+M_{11}M_{211}
+M_{11}M_{31}+\zeta_1^3M_3
\right.\\
&\left.
+\zeta_2M_3+M_{321}+\zeta_1M_{32}
\right)\\
&
+\zeta_2\ox\left(M_{41}
+\zeta_1M_{11}^2
+M_{11}M_3
+\zeta_1M_{31}
+M_5\right)
\end{align*}

\chapter*{}

\section{Algorithms for machine computations}

We finally briefly indicate how to use the obtained expressions to perform
actual calculations on a computer. Notably, knowledge of either a
multiplication map such as $A^\phi$ or of a comultiplication map such as
$A_\psi$ enables one to calculate all ordinary and matric triple Massey
product in the Steenrod algebra, as well as the $d_{(2)}$ differential of
the Adams spectral sequence, and hence its $E_3$ term --- see \cites{Baues,
Baues&JibladzeVI}.

\chapter*{}

We next utilize the quotient map $(\_)^{\le2}:\bar R_*\onto R_*^{\le2}$ given on the dual
monomial basis $M$ by sending all the elements $M_{n_1,...,n_k}$ with $k>2$ to
zero. Let us denote by $A_\psi^{\le2}$ the corresponding composite map
$$
\A_*\xto{A_\psi}\A_*\ox\bar R_*\onto\A_*\ox R_*^{\le2}
$$
Note that the composite
$$
\iota:\bar R_*\xto{(1\ox m^\r_*)m^\l_*=(m^\l_*\ox1)m^\r_*}\A_*\ox\bar
R_*\ox\A_*\onto\A_*\ox R_*^{\le2}\ox\A_*
$$
is injective --- the fact that we have used in \ref{L*} and \ref{S*} to
calculate the dual left action operator $L_*$ and the dual symmetry operator
$S_*$ respectively.

The equations \ref{apsi}\eqref{mreqs} and \eqref{mleqs} in particular imply that the composite
$$
W:\A_*\xto{A_\psi}\A_*\ox\bar R_*\xto{1\ox\iota}\A_*\ox\A_*\ox R_*^{\le2}\ox\A_*
$$
is determined by $A_\psi^{\le2}$; namely, one has
\begin{equation}\label{W}
W=
(m_*\ox1\ox1)(A_\psi^{\le2}\ox1)m_*
+(1\ox A_\psi^{\le2}\ox1)(1\ox m_*)m_*
+(1\ox1\ox(\_)^{\le2}\ox1)(1\ox m^\l_*\ox1)(\zeta_1\ox\bar b_\psi)m_*.
\end{equation}

We can now reformulate equations \ref{apsi}\eqref{mreqs} and \eqref{mleqs} in
terms of $A_\psi^{\le2}$. Indeed since the map $\iota$ is injective, these
equations are equivalent to the ones obtained by precomposing with the map
$1\ox\iota\ox1$, respectively $1\ox1\ox\iota$. Then using the equalities
$$
(\iota\ox 1)m^\r_*=(1\ox1\ox m_*)\iota
$$
for \eqref{mreqs} and
$$
(1\ox\iota)m^\l_*=(m_*\ox1\ox1)\iota
$$
for \eqref{mleqs}, we can prepend all occurrences of $A_\psi$ with
$1\ox\iota$, i.~e. switch from $A_\psi$ to $W$. In this way we arrive at the
equations
$$
(1\ox1\ox1\ox m_*)W=(W\ox1)m_*+(1\ox\iota\ox1)(\zeta_1\ox\bar b_\psi)m_*
$$
and
$$
(1\ox m_*\ox1\ox1)W=(m_*\ox1\ox1\ox1)W+(1\ox W)m_*,
$$
respectively. Next substituting here the values from \eqref{W} we obtain the
following equations on $A_\psi^{\le2}$:
\begin{multline*}
(1\ox1\ox1\ox m_*)(m_*\ox1\ox1)(A_\psi^{\le2}\ox1)m_*
+(1\ox1\ox1\ox m_*)(1\ox A_\psi^{\le2}\ox1)(1\ox m_*)m_*\\
+(1\ox1\ox1\ox m_*)(1\ox1\ox(\_)^{\le2}\ox1)(1\ox m^\l_*\ox1)(\zeta_1\ox\bar
b_\psi)m_*\\
=(m_*\ox1\ox1\ox1)(A_\psi^{\le2}\ox1\ox1)(m_*\ox1)m_*
+(1\ox A_\psi^{\le2}\ox1\ox1)(1\ox m_*\ox1)(m_*\ox1)m_*\\
+(1\ox1\ox(\_)^{\le2}\ox1\ox1)(1\ox m^\l_*\ox1\ox1)(\zeta_1\ox\bar
b_\psi\ox1)(m_*\ox1)m_*
\end{multline*}
and
\begin{multline*}
(1\ox m_*\ox1\ox1)(m_*\ox1\ox1)(A_\psi^{\le2}\ox1)m_*
+(1\ox m_*\ox1\ox1)(1\ox A_\psi^{\le2}\ox1)(1\ox m_*)m_*\\
+(1\ox m_*\ox1\ox1)(1\ox1\ox(\_)^{\le2}\ox1)(1\ox m^\l_*\ox1)(\zeta_1\ox\bar b_\psi)m_*\\
=
(m_*\ox1\ox1\ox1)(m_*\ox1\ox1)(A_\psi^{\le2}\ox1)m_*
+(m_*\ox1\ox1\ox1)(1\ox A_\psi^{\le2}\ox1)(1\ox m_*)m_*\\
+(m_*\ox1\ox1\ox1)(1\ox1\ox(\_)^{\le2}\ox1)(1\ox m^\l_*\ox1)(\zeta_1\ox\bar b_\psi)m_*
+(1\ox m_*\ox1\ox1)(1\ox A_\psi^{\le2}\ox1)(1\ox m_*)m_*\\
+(1\ox1\ox A_\psi^{\le2}\ox1)(1\ox1\ox m_*)(1\ox m_*)m_*
+(1\ox1\ox1\ox(\_)^{\le2}\ox1)(1\ox1\ox m^\l_*\ox1)(1\ox\zeta_1\ox\bar
b_\psi)(1\ox m_*)m_*.
\end{multline*}
It is straightforward to check that these equations are identically satisfied
for any choice of values for $A_\psi^{\le2}$.

In particular, for the values on the Milnor generators one has
\begin{multline*}
(1\ox\iota)A_\psi(\zeta_n)
=\sum_{0\le i\le n}(m_*\ox1)A_\psi^{\le2}(\zeta_{n-i}^{2^i})\ox\zeta_i
+\sum_{0\le i+j\le n}\zeta_{n-i-j}^{2^{i+j}}\ox A_\psi^{\le2}(\zeta_i^{2^j})\ox\zeta_j\\
+\sum_{0\le i\le n}\zeta_1\zeta_{n-i}^{2^i}\ox(1\ox(\_)^{\le2}\ox1)(m^\l_*\ox1)(\bar b_\psi(\zeta_i)).
\end{multline*}
Taking into account \eqref{apsisq}, \ref{4=0} and \eqref{bpsibar}, we then have
\begin{equation}\label{ia}
\begin{aligned}
(1\ox\iota)A_\psi(\zeta_n)
=&(m_*\ox(\_)^{\le2})C_n\ox\zeta_1+(m_*\ox1)(A_\psi^{\le2}(\zeta_n))\ox1\\
&+\sum_{0<i\le n}\zeta_{n-i}^{2^i}\ox(1\ox(\_)^{\le2})C_i\ox\zeta_1
+\sum_{0\le i\le n}\zeta_{n-i}^{2^i}\ox A_\psi^{\le2}(\zeta_i)\ox1\\
&+\sum_{\substack{0\le i\le n\\0<j<i}}\zeta_1\zeta_{n-i}^{2^i}\ox(1\ox(\_)^{\le2})(m^\l_*(v_{i-j}^{2^{j-1}}))\ox\zeta_j,
\end{aligned}
\end{equation}
where we have denoted
$$
C_i=L_*(\zeta_{i-1},\zeta_{i-1})+{\nabla_\xi}_*(\zeta_{i-1},\zeta_{i-1})
\in(\A_*\ox\bar R_*)_{2^i-1},\ i=1,2,3,...
$$

We see from these equations that the elements $A_\psi(\zeta_n)\in\A_*\ox\bar
R_*$ actually belong to a smaller subspace $\A_*\ox R_Q$, where
$R_Q\subset\bar R_*$ is the subspace defined by the equality
$$
R_Q=\iota\1(\A_*\ox R^{\le2}_*\ox Q_*),
$$
with $Q_*\subset\A_*$ denoting the linear subspace spanned by the polynomial
generators $1,\zeta_1,\zeta_2,\zeta_3,...$.

We also note that there is a commutative diagram
$$
\xymatrix{
&\A_*\ox R^{\le2}_*\ox\A_*\ar[dr]^{\eps\ox1\ox\eps}\\
\bar R_*\ar[ur]^\iota\ar[rr]^{(\_)^{\le2}}&&R^{\le2}_*,
}
$$
where $\eps:\A_*\to\FF$ is the counit. Indeed the dual diagram just expresses
the trivial fact that applying the multiplication map $\alpha\ox
r\ox\beta\mapsto\alpha r\beta$ to the tensor $1\ox r\ox1\in\A\ox
R^{\le2}\ox\A$ gives the value of the inclusion $R^{\le2}\into\bar R$ on the
element $r$. Thus for any $r\in\bar R_*$ we have
$$
r^{\le2}=(\eps\ox1\ox\eps)\iota(r).
$$

It is convenient in these circumstances to pick the basis $B_*$ of the space
$\bar R_*$ dual to the preadmissible basis $B$ of $\bar R$ as described in
\ref{barr}. Recall that the latter basis consists of elements of the form
$\pi\alpha$ where $\alpha$ is an admissible monomial and $\pi$ is a
preadmissible relation, i.~e. has form $\Sq^{n_k}\cdots\Sq^{n_1}[n_0,n]$
where $[n_0,n]$ is an Adem relation, the monomial $\Sq^{n_k}\cdots\Sq^{n_1}$
is admissible and moreover $n_1\ge2n_0$. Thus the dual basis $B_*$ consists
of linear forms $(\pi\alpha)_*$ on $\bar R$ which take value $1$ on
$\pi\alpha$ and $0$ on all other elements of $B$. We will call $B_*$ the
\emph{dual preadmissible basis} of $\bar R_*$. It is convenient for us because
of the following

\begin{Lemma}
The dual preadmissible basis $B_*$ has the following properties:
\begin{itemize}
\item
the subset $B_Q$ of $B_*$ consisting of the elements
$(\pi1)_*$ and $(\pi\Sq^{2^k}\Sq^{2^{k-1}}\cdots\Sq^2\Sq^1)_*$ for all
preadmissible relations $\pi$ and all $k\ge0$ is a basis for the subspace
$R_Q$ of $\bar R_*$;
\item
the elements $(\pi1)_*$ for all preadmissible relations $\pi$ form a basis
$B_0$ of the subspace
$$
R_0=\iota\1(\A_*\ox R^{\le2}_*\ox\FF1)\subset R_Q\subset\bar R_*;
$$
\item
for each $k\ge1$ the elements $(\pi1)_*$ and
$(\pi\Sq^{2^j}\Sq^{2^{j-1}}\cdots\Sq^2\Sq^1)_*$ with $j<k$ form a basis $B_k$
of the subspace
$$
R_k=\iota\1\left(\bigoplus_{0\le j\le k}\A_*\ox
R^{\le2}_*\ox\FF\zeta_j\right)\subset R_Q\subset\bar R_*;
$$
\item
the map $(\_)^{\le2}:\bar R_*\to R^{\le2}_*$  sends the elements $(1[n,m]1)_*$ 
to $[n,m]_*$ and all other elements of $B_*$ to $0$.
\end{itemize}
\end{Lemma}

\begin{proof}

\end{proof}

Thus we have a filtration
$$
B_0\subset B_1\subset\cdots\subset B_Q\subset B_*;
$$
let us also single out the subset
$$
B_{\textrm{Adem}}\subset B_0
$$
consisting of the duals $[a,b]_*=(1[a,b]1)_*$ of the Adem relations, for
$0<a<2b$, $a,b\in\NN$.

With respect to the basis $B_Q$, any solution $A_\psi(\zeta_n)$ of the above
equation can be written in the form
$$
A_\psi(\zeta_n)=\sum_{\beta\in B_Q}X_{2^n-|\beta|}(\beta)\ox\beta,
$$
for some uniquely determined elements
$X_{2^n-|\beta|}(\beta)\in\A_{2^n-|\beta|}$, where $|\beta|$ denotes degree of
the (homogeneous) element $\beta$. Moreover in these terms one has
$$
A_\psi^{\le2}(\zeta_n)=\sum_{a<2b}X_{2^n-a-b}([a,b]_*)\ox[a,b]_*.
$$

\begin{comment}
When substituting these expressions in \eqref{ia} it will be also convenient
to use the map
$$
\tilde\iota:\bar R_*\to(\tilde\A_*\ox\bar R_*\ox\A_*+\A_*\ox\bar
R_*\ox\tilde\A_*)\subset\A_*\ox\bar R_*\ox\A_*
$$
determined by the equality
$$
\iota(r)=1\ox r\ox1+\tilde\iota(r).
$$
Note that the elements $\tilde\iota([a,b]_*)\in\tilde\A_*\ox R^{\le2}_*\ox\FF1$ are
not necessarily zero. For example, one has
\begin{align*}
\tilde\iota([1,3]_*)&=\zeta_1\ox[1,2]_*\ox1,\\
\tilde\iota([3,2]_*)&=\zeta_1\ox[2,2]_*\ox1,\\
\tilde\iota([1,5]_*)&=\zeta_1\ox([1,4]_*+[2,3]_*)\ox1,\\
\tilde\iota([3,3]_*)&=\zeta_1\ox[2,3]_*\ox1+\zeta_1^2\ox[2,2]_*\ox1,
\end{align*}
etc.
\end{comment}

Substituting this into \eqref{ia} one obtains
\begin{align*}
\sum_{\beta\in B_Q}X_{2^n-|\beta|}(\beta)\ox\iota\beta
&=\sum_{a<2b}
\left(
m_*(X_{2^n-a-b}([a,b]_*))+\sum_{0\le i\le n}\zeta_{n-i}^{2^i}\ox X_{2^i-a-b}([a,b]_*)\right)
\ox[a,b]_*\ox1\\
&+\left((m_*\ox(\_)^{\le2})C_n
+\sum_{0<i\le n}\zeta_{n-i}^{2^i}\ox(1\ox(\_)^{\le2})C_i
+\sum_{1\le i\le n}\zeta_1\zeta_{n-i}^{2^i}\ox(1\ox(\_)^{\le2})(m^\l_*(v_{i-1}))
\right)\ox\zeta_1\\
&+\sum_{j\ge2}\left(\sum_{j<i\le
n}\zeta_1\zeta_{n-i}^{2^i}\ox(1\ox(\_)^{\le2})(m^\l_*(v_{i-j}^{2^{j-1}}))\right)\ox\zeta_j
\end{align*}

Moreover let us write for $\beta\in B_Q$
$$
\iota\beta=\sum_{k\ge0}c_{|\beta|-2^k+1}(\beta)\ox\zeta_k
$$
with $c_j(\beta)\in(\A_*\ox R^{\le2}_*)_j$ the \emph{coordinates} of $\beta$.
\begin{comment}
Thus we have
$$
\tilde\iota\beta=\tilde c_{|\beta|}(\beta)\ox1+\sum_{k\ge1}c_{|\beta|-2^k+1}(\beta)\ox\zeta_k,
$$
where
$$
c_{|\beta|}(\beta)=1\ox\beta+\tilde c_{|\beta|}(\beta),
$$
with $\tilde c_{|\beta|}(\beta)\in(\tilde\A_*\ox R^{\le2}_*)_{|\beta|}$.
\end{comment}

Then collecting terms with respect to the last component, the above equation
becomes equivalent to the system
$$
\left\{
\begin{aligned}
\sum_{\beta\in B_Q}X_{2^n-|\beta|}(\beta)\ox c_{|\beta|}(\beta)
&=\sum_{a<2b}
\left(
m_*(X_{2^n-a-b}([a,b]_*))
+\sum_{0\le i\le n}\zeta_{n-i}^{2^i}\ox X_{2^i-a-b}([a,b]_*)
\right)
\ox[a,b]_*,\\
\sum_{\beta\in B_Q-B_0}X_{2^n-|\beta|}(\beta)\ox c_{|\beta|-1}(\beta)
&=(m_*\ox(\_)^{\le2})C_n
+\sum_{0<i\le n}\zeta_{n-i}^{2^i}\ox(1\ox(\_)^{\le2})C_i\\
&+\sum_{1<i\le n}\zeta_1\zeta_{n-i}^{2^i}\ox(1\ox(\_)^{\le2})(m^\l_*(v_{i-1})),\\
\sum_{\beta\in B_Q-B_j}X_{2^n-|\beta|}(\beta)\ox c_{|\beta|-2^j+1}(\beta)
&=\sum_{j<i\le
n}\zeta_1\zeta_{n-i}^{2^i}\ox(1\ox(\_)^{\le2})(m^\l_*(v_{i-j}^{2^{j-1}})),&j\ge2.
\end{aligned}
\right.
$$

\endinput

